A Computational Framework for Solving Wasserstein Lagrangian Flows

The dynamical formulation of the optimal transport can be extended through various choices of the underlying geometry (kinetic energy), and the regularization of density paths (potential energy). These combinations yield different variational problems (Lagrangians), encompassing many variations of the optimal transport problem such as the Schr\"odinger bridge, unbalanced optimal transport, and optimal transport with physical constraints, among others. In general, the optimal density path is unknown, and solving these variational problems can be computationally challenging. We propose a novel deep learning based framework approaching all of these problems from a unified perspective. Leveraging the dual formulation of the Lagrangians, our method does not require simulating or backpropagating through the trajectories of the learned dynamics, and does not need access to optimal couplings. We showcase the versatility of the proposed framework by outperforming previous approaches for the single-cell trajectory inference, where incorporating prior knowledge into the dynamics is crucial for correct predictions.

==> text/03_computation.tex <==
\subsection{Computational Approach for Solving Wasserstein Lagrangian Flows}\label{sec:computational}

In this section, we describe our computational approach to solving for Wasserstein Lagrangian Flows, which proceeds in two steps corresponding to the inner and outer optimizations in \cref{eq:dual_intermediate}. 
We first consider how to \textbf{\textit{evaluate}} %(\cref{sec:eval}) 
the action functional $\cA_{\cL}[\qm_t]$ for a given curve $\qm_t$, then propose an efficient method to \textbf{\textit{optimize}} the action over curves $\qm_t \in \mmarginalcouple$ satisfying the desired constraints.   
We restrict attention to Lagrangian optimizations with linearizable objectives as in \cref{def:dual_linearizable} and maintain separate parameterizations of the cotangent vector $\lagr_t$ and distributional path $\qm_t$ in all cases.  We summarize our algorithm in \cref{algorithm:wlm}.

\subsubsection{Evaluating $\cA_{\cL}[\qm_t]$ using Action Matching:}\label{sec:eval}
%\paragraph{Evaluating $\cA_{\cL}[\qm_t]$ using Action Matching:}
Returning to the action-minimization problem in \cref{prop:dual_obj}, consider the problem of evaluating action functional $\cA_{\cL}[\qm_t]$ for a given $\qm_t \in \mmarginalcouple$.   
For a dual linearizable Lagrangian in \cref{def:dual_linearizable}, the action in \cref{eq:action} is given by
%\small
\begin{equation}
%\label{eq:dual_general} 
%\nonumber
\hspace*{-.22cm} \cA_{\cL}[\qm_t]=  \sup \limits_{\lagr_t}  \int \lagr_1 \mu_1 dx_1 -  \int \lagr_0 \mu_0 dx_0  -\int_0^1\int \left( \frac{\partial \lagr_t }{\partial t} + K^*[x_t, \lagr_t, t] + U[x_t, \lagr_t, t] \right) \qm_t dx_t dt. \label{eq:am_general}
\end{equation}
\normalsize
%We treat the \gls{AM} optimization over $\lagr_t$ as an inner loop to evaluate $\cA_{\cL}[\qm_t]$ at each step in the optimization.
% \paragraph{Parameterization}
% Noting that cotangent vectors 
%  parameterize $\lagr_t$ as a neural network $\lagr_t(x,\theta)$ which takes $t$ and $x$ as inputs with parameters $\theta$.
% \paragraph{Relationship with Action Matching} 
We can immediately recognize the similarity of this objective to the \gls{AM} objective in \cref{eq:action_matching}, suggesting that 
Action Matching can be viewed as an inner loop to evaluate $\cA_{\cL}[\qm_t]$ for each curve $\qm_t$ in the outer optimization of \cref{prop:dual_obj}.  
The optimal cotangent vectors $\lagr_{\dot{\qm}_t}$ correspond to the tangent vectors $\dot{\qm}_t$ of the given curve via the Legendre transform in \cref{eq:l_legendre}.

\paragraph{Parameterization}  We parameterize $\lagr_t : \cX \times [0,1] \rightarrow \bbR$ as a neural network $\lagr_t(x,\theta)$ with parameters $\theta$,  which takes $t$ and $x$ as input and outputs a scalar (see \cref{eq:dual_for_optimization} below).


\paragraph{Relationship with Action Matching} \RB{Defer to Related Work?   Is the statement above `AM as Inner Loop' convincing enough?}
\citet{neklyudov2023action} assume access to samples from a \textit{continuous} curve of densities $\mu_{t}$, which corresponds to the limit as the number of constraints $M \rightarrow \infty$.   Translating this case to our framework, the outer optimization over $\qm_t$ can be ignored since $\qm_t \in \mmarginalcouple$ has no remaining degrees of freedom, and expectations in \cref{eq:action_matching} are written directly under $\mu_t$.
However, the assumption of a continuous density path is unreasonable in practical applications such as trajectory inference, where data is sampled discretely in time.  In this setting, our outer optimization 
$\cS_\cL(\{\mu_{t_i}\}) = \inf_{\qm_t} \cA_{\cL}[\qm_t]$ over curves $\qm_t \in \marginalcouple$ 
is necessary to \textit{interpolate} between $M$ given marginals using the inductive bias encoded in the Lagrangian $\cL[\qm_t, \dot{\qm}_t, t]$.   



% Recognizing the similarity of this objective to the \gls{AM} objective in \cref{eq:action_matching}, 
% we consider Action Matching as an inner loop to evaluate $\cA_{\cL}[\qm_t]$ for each candidate curve in the optimization in \cref{eq:} 

%We can immediately recognize the inner optimization as having the same form as the Action Matching objective in \cref{eq:action_matching}.     
%We treat the \gls{AM} optimization over $\lagr_t$ as an inner loop to evaluate $\cA_{\cL}[\qm_t]$ at each step in the optimization.  


%where our physical potentials in Hamiltonian 

  





% \paragraph{Relationship with Action Matching} 
% The objective in \cref{eq:dual_intermediate} is reminiscent of the \gls{AM} framework \citep{neklyudov2023action} for various choices of $\cH[\qm_t, \lagr_t, t]$.   Only the inner optimization over $\lagr_t$ is performed in \gls{AM}, since an absolutely continuous curve $\mu_t \in \marginalcouple$ is assumed to be given as a dataset, with the number of marginal constraints $M \rightarrow \infty$.
% % limit as M \rightarrow \infty.  
% This assumption may be unreasonable in practical applications such as trajectory inference, where data is sampled discretely in time. 
% In our setting, the outer optimization over $\qm_t \in \marginalcouple$ is necessary to find the optimal curve of interpolating marginals, as specified by \hl{(the prior information in)} the Lagrangian $\cL[\qm_t, \dot{\qm}_t, t]$,
% with the Action Matching optimization over $\lagr_t$ as an inner loop.

% %\paragraph{Relationship with Dynamical Formulations} argue why this is better than \RB{Remark 10}:  holds for any Hamiltonian, including nonlinear.   reference appendix.  (or let this be the intro to \cref{sec:linearize})

\subsubsection{Optimizing over Constrained Curves}\label{sec:parametrization}

Inspired by the fact that we only need to draw samples from $\qm_t$ for linearizable objectives in \cref{def:dual_linearizable},
%potential energies , 
we parameterize the distribution path $\qm_t(x,\eta)$ as a generative model, where the samples are generated as follows










\hl{Nevertheless, upon reaching an optimal $\qm_t$, our primary object of interest is the dynamics model corresponding to $\dot{\qm}_t$ and parameterized by the optimal $\lagr_{\dot{\qm}_t}$ from \cref{eq:l_legendre} or (\cref{eq:am_general}), which may be used to run simulations and make predictions at the level of individual trajectories.}


%\subsubsection{Parameterization and Optimization}\label{sec:parametrization}


% For any Lagrangian optimization with a linearizable objective as in \cref{def:dual_linearizable}, we consider
% 5We consider 
% parameterizing the cotangent vectors $\lagr_t$ and the distributional path $\qm_t$, %However, as mentioned above, we restrict 
% % restricting attention to potential energies which admit a dual which is linear in $\qm_t$ as in \cref{def:dual_linearizable}.
% We parameterize $\lagr_t$ as a neural network $\lagr_t(x,\theta)$ which takes $t$ and $x$ as inputs with parameters $\theta$, and outputs a scalar.
Inspired by the fact that we only need to draw samples from $\qm_t$ for these problems,
%potential energies with linearizable objectives as in \cref{def:dual_linearizable}, 
we parameterize the distribution path $\qm_t(x,\eta)$ as a generative model, where the samples are generated as follows
% For these cases, we propose a parameterization inspired by the fact that we only need to draw samples from $\qm_t$ and need not evaluate its density.
% We consider objectives of the following type
% \begin{align}
% \cS&(\cL, \{\mu_{0,1}\}) = \sup \limits_{\lagr_t} \inf \limits_{\qm_t} ~ \int \lagr_1 d\mu_1 -  \int \lagr_0 d\mu_0 -\int_0^1\int U[\lagr_t]\qm_t dx_t dt, 
% \end{align}
% where $U[\lagr_t]$ represents Hamilton-Jacobi equation.
%In particular, We parameterize the distribution path $\qm_t(x,\eta)$ as a generative model, where the samples are generated as follows
\begin{align}
    x_t = (1-t)x_0 + tx_1 + t(1-t)\textsc{nnet}(t,x_0,x_1,\eta), \;\; x_0 \sim \mu_0, \;\; x_1 \sim \mu_1.
\end{align}
Notably, this preserves the endpoint marginals $\mu_0, \mu_1$. 
For multiple constraints, we can modify our sampling procedure to interpolate between two intermediate dataset marginals, with neural network parameters $\eta$ shared across timesteps
\small
% \frac{t_{i+1}-t}{t_{i+1}-t_i} \frac{t-t_{i}}{t_{i+1}-t_i}
\begin{align}
    x_t = \frac{t_{i+1}-t}{t_{i+1}-t_i} x_{t_i} + \frac{t-t_{i}}{t_{i+1}-t_i} x_{t_{i+1}} + 
    \left(1- \left(\frac{t_{i+1}-t}{t_{i+1}-t_i}\right)^2 - \left(\frac{t-t_{i}}{t_{i+1}-t_i}\right)^2\right)\textsc{nnet}(t,x_{t_i},x_{t_{i+1}},\eta)\,.
    \nonumber
\end{align}
\normalsize
which ensures $\qm_t \in \mmarginalcouple$ as desired in \cref{prop:dual_obj}.
Our overall optimization objective becomes
%For dual objectives as in \cref{{eq:dual_intermediate}} and \cref{eq:am_general}, we optimize
% \small
\begin{align}
\textsc{loss}(\theta, \eta) =  \min \limits_{\eta}\max \limits_{\theta} &\int \lagr_1(x,\theta) d\mu_1 -  \int \lagr_0(x,\theta) d\mu_0 \label{eq:dual_for_optimization} \\
- \int_0^1 &\int 
\left( \frac{\partial \lagr_t}{\partial t}(x,\theta) + K^*[\lagr_t(x,\theta), t] + U[\lagr_t(x,\theta), t] \right)
%\hj[\lagr_t(x,\theta)]
\qm_t(x,\eta)dx dt,  \nonumber
\end{align}
\normalsize
where the optimization w.r.t. $\eta$ is performed via the re-parameterization trick.
An alternative to parametrizing the distributional path $\qm_t$ is the minimization of 
\cref{eq:dual_general}
%\cref{eq:dual_for_optimization}
via the Wasserstein gradient flow, i.e. the samples $x_t$ from the initial path $\qm_t$ are updated as follows
\begin{align}
    x_t' = x_t + \alpha \cdot t (1-t)\nabla_x \left[\frac{\partial \lagr_t}{\partial t}(x_t,\theta) + K^*[\lagr_t(x_t,\theta), t] + U[\lagr_t(x_t,\theta), t]\right]\,,
\end{align}
where $\alpha$ is a hyperparameter regulating the step-size, and the coefficient $t(1-t)$ guarantees the preservation of marginals. 
In practice, we find that combining both 
the parametric and nonparametric
approaches works best.
The pseudo-code for the resulting algorithm is given in \cref{algorithm:wlm}. 



\vheader
\paragraph{Discontinuous Interpolation}
\vheader
The support of the optimal distribution path $\qm_t$ might be disconnected, as in \cref{fig:examples_a}.
Thus, it may be impossible to interpolate continuously between independent
%ly drawn 
samples from the marginals while staying in the support of the optimal path.
To allow for a discontinuous interpolation, we pass a discontinuous indicator variable $\mathbbm{1}[t < 0.5]$ to the model $\qm_t(x,\eta)$.
\vheader




==> text/03_param.tex <==
\vheader
\vheader
\subsection{Parameterization and Optimization}\label{sec:parametrization}
\vheader

\setlength{\textfloatsep}{10pt}
% \resizebox{0.9\textwidth}{!}{
% \begin{minipage}{\linewidth}
\begin{algorithm}[t]
%\scriptsize
\footnotesize
  \begin{algorithmic}
    \caption{Learning Wasserstein Lagrangian Flows}\label{algorithm:wlm}
    \REQUIRE samples from the marginals $\mu_0, \mu_1$, parametric model $\lagr_t(x,\theta)$, generator from $\qm_t(x,\eta)$
    \FOR{learning iterations}
        \STATE sample from marginals $\{x_0^i\}_{i=1}^n \sim \mu_0, \; \{x_1^i\}_{i=1}^n \sim \mu_1$, sample time $\{t^i\}_{i=1}^n \sim \textsc{uniform}[0,1]$
        \STATE $x_t^i = (1-t^i)x_0^i + t^ix_1^i + t^i(1-t^i)\textsc{nnet}(t^i,x_0^i,x_1^i,\eta)$
        \STATE $\textsc{grad}_\eta = -\nabla_\eta \frac{1}{n}\sum_i^n\left[\frac{\partial \lagr_{t^i}}{\partial t^i}(x_t^i(\eta),\theta) + K^*[\lagr_t(x_t^i(\eta),\theta), t^i] + U[\lagr_{t^i}(x_t^i(\eta),\theta), t^i]\right]$
        \FOR{Wasserstein gradient steps}
        \STATE $x_t^i \gets x_t^i + \alpha \cdot t^i (1-t^i)\nabla_x \left[\frac{\partial \lagr_{t^i}}{\partial t^i}(x_t^i,\theta) + K^*[\lagr_{t^i}(x_t^i,\theta), t^i] + U[\lagr_{t^i}(x_t^i,\theta), t^i]\right]$
        \ENDFOR
        \STATE $\textsc{grad}_\theta = \nabla_\theta \frac{1}{n}\sum_{i}^n\left[\lagr_1(x_1^i,\theta) - \lagr_0(x_0^i,\theta) - \frac{\partial \lagr_{t^i}(x_t^i,\theta)}{\partial t^i} - K^*[\lagr_{t^i}(x_t^i,\theta), t^i] - U[\lagr_{t^i}(x_t^i,\theta), t^i]\right]$
        \STATE update parameters using gradients $\textsc{grad}_\eta, \textsc{grad}_\theta$
    \ENDFOR
    \RETURN cotangent vectors $\lagr_t(x,\theta)$
  \end{algorithmic}
\end{algorithm}
%\end{minipage}
%}
For each problem, we consider parameterizing the cotangent vectors $\lagr_t$ and the distributional path $\qm_t$, %However, as mentioned above, we restrict 
restricting attention to potential energies which admit a dual which is linear in $\qm_t$ as in \cref{def:dual_linearizable}.
%\cref{eq:linear_dual}.  
For these cases, we propose a parameterization inspired by the fact that we only need to draw samples from $\qm_t$ and need not evaluate its density.
% We consider objectives of the following type
% \begin{align}
% \cS&(\cL, \{\mu_{0,1}\}) = \sup \limits_{\lagr_t} \inf \limits_{\qm_t} ~ \int \lagr_1 d\mu_1 -  \int \lagr_0 d\mu_0 -\int_0^1\int U[\lagr_t]\qm_t dx_t dt, 
% \end{align}
% where $U[\lagr_t]$ represents Hamilton-Jacobi equation.
In particular, we parameterize $\lagr_t$ as a neural network $\lagr_t(x,\theta)$ which takes $t$ and $x$ as inputs with parameters $\theta$.
We parameterize the distribution path $\qm_t(x,\eta)$ as a generative model, where the samples are generated as follows
\begin{align}
    x_t = (1-t)x_0 + tx_1 + t(1-t)\textsc{nnet}(t,x_0,x_1,\eta), \;\; x_0 \sim \mu_0, \;\; x_1 \sim \mu_1.
\end{align}
Notably, this preserves the endpoint marginals $\mu_0, \mu_1$.   For dual objectives as in \cref{{eq:dual_general}}, we optimize
% \small
\begin{align}
\textsc{loss}(\theta, \eta) = \max \limits_{\theta} \min \limits_{\eta} &\int \lagr_1(x,\theta) d\mu_1 -  \int \lagr_0(x,\theta) d\mu_0 \label{eq:dual_for_optimization} \\
- \int_0^1 &\int 
\left( \frac{\partial \lagr_t}{\partial t}(x,\theta) + K^*[\lagr_t(x,\theta), t] + U[\lagr_t(x,\theta), t] \right)
%\hj[\lagr_t(x,\theta)]
\qm_t(x,\eta)dx dt,  \nonumber
\end{align}
\normalsize
where the optimization w.r.t. $\eta$ is performed via the re-parameterization trick.
An alternative to parametrizing the distributional path $\qm_t$ is the minimization of 
\cref{eq:dual_general}
%\cref{eq:dual_for_optimization}
via the Wasserstein gradient flow, i.e. the samples $x_t$ from the initial path $\qm_t$ are updated as follows
\begin{align}
    x_t' = x_t + \alpha \cdot t (1-t)\nabla_x \left[\frac{\partial \lagr_t}{\partial t}(x_t,\theta) + K^*[\lagr_t(x_t,\theta), t] + U[\lagr_t(x_t,\theta), t]\right]\,,
\end{align}
where $\alpha$ is a hyperparameter regulating the step-size, and the coefficient $t(1-t)$ guarantees the preservation of marginals. 
In practice, we find that combining both 
the parametric and nonparametric
approaches works best.
The pseudo-code for the resulting algorithm is given in \cref{algorithm:wlm}. 
\vheader
\paragraph{Discontinuous Interpolation}
\vheader
The support of the optimal distribution path $\qm_t$ might be disconnected, as in \cref{fig:examples_a}.
Thus, it may be impossible to interpolate continuously between independent
%ly drawn 
samples from the marginals while staying in the support of the optimal path.
To allow for a discontinuous interpolation, we pass a discontinuous indicator variable $\mathbbm{1}[t < 0.5]$ to the model $\qm_t(x,\eta)$.
\vheader

\vheader
\paragraph{Handling Multiple Marginal Constraints}%\label{sec:multiple_marginals}
\vheader
While we have only considered endpoint marginal constraints in our examples so far, we can also incorporate intermediate marginal constraints for any of the problems above. 
For example, for a time-evolving system sampled discretely in time, we might enforce that our sampling distribution match the marginals $\mu_{t_i}$ given by the dataset.  
%Such examples are prevalent in trajectory inference problems in biological applications \citep{schiebinger2019optimal, tong2023conditional}.
Introducing Lagrange multipliers for each intermediate marginal constraint in \cref{eq:general_lagr_min}, we obtain
\RB{FIX ORDERING HERE?}
\scriptsize
\begin{align}%\label{eq:multi-marginal}
\hspace{-.1cm} 
%\cS_{\cL}&(\{\mu_{t_i}\}) = 
\sup \limits_{\lagr_t, \lambda_{t_i}} \inf \limits_{\qm_t} ~ \int \lagr_1 \mu_1 dx_1 -  \int \lagr_0 \mu_0 dx_0 
+ \sum \limits_{i=1}^{M-2} \int  \lambda_{t_i} \big(  \mu_{t_i} - \qm_{t_i} \big)   dx_{t_i}  
%\\
%&\phantom{(\cL, \{\}=}
-\int_0^1  \int  
\left(\frac{\partial \lagr_t}{\partial t} + K^*[x_t,\lagr_t] + U[x_t,\lagr_t]
%\hj[ \lagr_t, x_t] 
\right)
 \qm_t dx_t dt.  \nonumber
\end{align}
\normalsize
To handle multiple marginal constraints, we simply modify our sampling procedure to interpolate between two intermediate dataset marginals, with neural network parameters $\eta$ shared across timesteps
\small
% \frac{t_{i+1}-t}{t_{i+1}-t_i} \frac{t-t_{i}}{t_{i+1}-t_i}
\begin{align}
    x_t = \frac{t_{i+1}-t}{t_{i+1}-t_i} x_{t_i} + \frac{t-t_{i}}{t_{i+1}-t_i} x_{t_{i+1}} + 
    \left(1- \left(\frac{t_{i+1}-t}{t_{i+1}-t_i}\right)^2 - \left(\frac{t-t_{i}}{t_{i+1}-t_i}\right)^2\right)\textsc{nnet}(t,x_{t_i},x_{t_{i+1}},\eta)\,,
    \nonumber
\end{align}
\normalsize
% \small
% % \frac{t_{i+1}-t}{t_{i+1}-t_i} \frac{t-t_{i}}{t_{i+1}-t_i}
% \begin{align}
%     x_t = \frac{t_{i+1}-t}{t_{i+1}-t_i} x_{t_i} + \frac{t-t_{i}}{t_{i+1}-t_i} x_{t_{i+1}} + 
%     \Big(1- \big(\frac{t_{i+1}-t}{t_{i+1}-t_i}\big)^2 - \big(\frac{t-t_{i}}{t_{i+1}-t_i}\big)^2\Big)\textsc{nnet}(t,x_{t_i},x_{t_{i+1}},\eta)\,,
%     \nonumber
% \end{align}
% \normalsize
where $x_{t_i} \sim \mu_{t_i}$ and $x_{t_{i+1}} \sim \mu_{t_{i+1}}$.
Note that since $\qm_{t_i} = \mu_{t_i}$ by construction, we do not need to optimize the intermediate Lagrange multiplier terms above.   See \cref{app:multiple-marginal} for further discussion.
%\hl{At optimality, our procedure will recover the solution to a concatenation of Lagrangian flows between neighboring marginals $\{ \mu_0, \mu_{t_1}\}, ... \{  \mu_{t_{M-2}}, \mu_{1} \}$ }, as discussed in \cref{app:}.


% To see this, note that the concatenation of dual objectives for $M=3$, or action-minimization problems between $\{\mu_{0,t_1}\}$ and $\{\mu_{t_1,1}\}$ yields 
% %a dual objective where intermediate potentials.
% %cancel $\cS_{\cL}(\{\mu_{0,t_1}\}) + \cS_{\cL}(\{\mu_{t_1,1}\}) =  $
% the 
% following dual objective
% \small
% \begin{align}
% \begin{split}
%     \cS_{\cL}(\{\mu_{0,t_1}\}) + \cS_{\cL}(\{\mu_{t_1,1}\}) &= \sup \limits_{\lagr_t} \inf \limits_{\qm_t} ~ \int \lagr_{t_1} d\mu_{t_1} -  \int \lagr_0 d\mu_0 +\int_0^{t_1}  \int  \left(\frac{\partial \lagr_t}{\partial t} + K[\lagr_t] + U[\lagr_t]\right) ~ \qm_t dx_t dt \\ & + \sup \limits_{\lagr_t} \inf \limits_{\qm_t} ~ \int \lagr_{1} d\mu_{1}  -  \int \lagr_{t_1} d\mu_{t_1} +\int_{t_1}^1  \int  
%     \left(\frac{\partial \lagr_t}{\partial t} + K[\lagr_t] + U[\lagr_t]\right)
%     %\hj[ \lagr_t, x_t] 
%     ~ \qm_t dx_t dt 
% \end{split}\nonumber
% \end{align}
% \normalsize
% which matches \cref{eq:multi-marginal} after telescoping cancellation and removing the Lagrange multipliers as justified above.

% \vspace{-35pt}
%\vspace*{-.2cm}
%\begin{center*}
%
% \vspace{-35pt}

%\end{center*}

==> text/03_param_new.tex <==
\subsection{Parameterization and Optimization}\label{sec:parametrization}
\vheader

\setlength{\textfloatsep}{10pt}
% \resizebox{0.9\textwidth}{!}{
% \begin{minipage}{\linewidth}
\begin{algorithm}[t]
%\scriptsize
\footnotesize
  \begin{algorithmic}
    \caption{Learning Wasserstein Lagrangian Flows}\label{algorithm:wlm}
    \REQUIRE samples from the marginals $\mu_0, \mu_1$, parametric model $\lagr_t(x,\theta)$, generator from $\qm_t(x,\eta)$
    \FOR{learning iterations}
        \STATE sample from marginals $\{x_0^i\}_{i=1}^n \sim \mu_0, \; \{x_1^i\}_{i=1}^n \sim \mu_1$, sample time $\{t^i\}_{i=1}^n \sim \textsc{uniform}[0,1]$
        \STATE $x_t^i = (1-t^i)x_0^i + t^ix_1^i + t^i(1-t^i)\textsc{nnet}(t^i,x_0^i,x_1^i,\eta)$
        \STATE $\textsc{grad}_\eta = -\nabla_\eta \frac{1}{n}\sum_i^n\left[\frac{\partial \lagr_{t^i}}{\partial t^i}(x_t^i(\eta),\theta) + K^*[\lagr_t(x_t^i(\eta),\theta), t^i] + U[\lagr_{t^i}(x_t^i(\eta),\theta), t^i]\right]$
        \FOR{Wasserstein gradient steps}
        \STATE $x_t^i \gets x_t^i + \alpha \cdot t^i (1-t^i)\nabla_x \left[\frac{\partial \lagr_{t^i}}{\partial t^i}(x_t^i,\theta) + K^*[\lagr_{t^i}(x_t^i,\theta), t^i] + U[\lagr_{t^i}(x_t^i,\theta), t^i]\right]$
        \ENDFOR
        \STATE $\textsc{grad}_\theta = \nabla_\theta \frac{1}{n}\sum_{i}^n\left[\lagr_1(x_1^i,\theta) - \lagr_0(x_0^i,\theta) - \frac{\partial \lagr_{t^i}(x_t^i,\theta)}{\partial t^i} - K^*[\lagr_{t^i}(x_t^i,\theta), t^i] - U[\lagr_{t^i}(x_t^i,\theta), t^i]\right]$
        \STATE update parameters using gradients $\textsc{grad}_\eta, \textsc{grad}_\theta$
    \ENDFOR
    \RETURN cotangent vectors $\lagr_t(x,\theta)$
  \end{algorithmic}
\end{algorithm}
%\end{minipage}
%}
For each problem, we consider parameterizing the cotangent vectors $\lagr_t$ and the distributional path $\qm_t$, %However, as mentioned above, we restrict 
restricting attention to potential energies which admit a dual which is linear in $\qm_t$ as in \cref{def:dual_linearizable}.
%\cref{eq:linear_dual}.  
For these cases, we propose a parameterization inspired by the fact that we only need to draw samples from $\qm_t$ and need not evaluate its density.
% We consider objectives of the following type
% \begin{align}
% \cS&(\cL, \{\mu_{0,1}\}) = \sup \limits_{\lagr_t} \inf \limits_{\qm_t} ~ \int \lagr_1 d\mu_1 -  \int \lagr_0 d\mu_0 -\int_0^1\int U[\lagr_t]\qm_t dx_t dt, 
% \end{align}
% where $U[\lagr_t]$ represents Hamilton-Jacobi equation.
In particular, we parameterize $\lagr_t$ as a neural network $\lagr_t(x,\theta)$ which takes $t$ and $x$ as inputs with parameters $\theta$.
We parameterize the distribution path $\qm_t(x,\eta)$ as a generative model, where the samples are generated as follows
\begin{align}
    x_t = (1-t)x_0 + tx_1 + t(1-t)\textsc{nnet}(t,x_0,x_1,\eta), \;\; x_0 \sim \mu_0, \;\; x_1 \sim \mu_1.
\end{align}
Notably, this preserves the endpoint marginals $\mu_0, \mu_1$.   For dual objectives as in \cref{{eq:dual_general}}, we optimize
% \small
\begin{align}
\textsc{loss}(\theta, \eta) = \max \limits_{\theta} \min \limits_{\eta} &\int \lagr_1(x,\theta) d\mu_1 -  \int \lagr_0(x,\theta) d\mu_0 \label{eq:dual_for_optimization} \\
- \int_0^1 &\int 
\left( \frac{\partial \lagr_t}{\partial t}(x,\theta) + K^*[\lagr_t(x,\theta), t] + U[\lagr_t(x,\theta), t] \right)
%\hj[\lagr_t(x,\theta)]
\qm_t(x,\eta)dx dt,  \nonumber
\end{align}
\normalsize
where the optimization w.r.t. $\eta$ is performed via the re-parameterization trick.
An alternative to parametrizing the distributional path $\qm_t$ is the minimization of 
\cref{eq:dual_general}
%\cref{eq:dual_for_optimization}
via the Wasserstein gradient flow, i.e. the samples $x_t$ from the initial path $\qm_t$ are updated as follows
\begin{align}
    x_t' = x_t + \alpha \cdot t (1-t)\nabla_x \left[\frac{\partial \lagr_t}{\partial t}(x_t,\theta) + K^*[\lagr_t(x_t,\theta), t] + U[\lagr_t(x_t,\theta), t]\right]\,,
\end{align}
where $\alpha$ is a hyperparameter regulating the step-size, and the coefficient $t(1-t)$ guarantees the preservation of marginals. 
In practice, we find that combining both 
the parametric and nonparametric
approaches works best.
The pseudo-code for the resulting algorithm is given in \cref{algorithm:wlm}. 


\vheader
\paragraph{Handling Multiple Marginal Constraints}%\label{sec:multiple_marginals}
\vheader
While we have only considered endpoint marginal constraints in our algorithm so far, we can also easily incorporate multiple marginal constraints in marginal-preserving fashion.
In particular, we modify our sampling procedure to interpolate between two intermediate dataset marginals, with neural network parameters $\eta$ shared across timesteps
\small
% \frac{t_{i+1}-t}{t_{i+1}-t_i} \frac{t-t_{i}}{t_{i+1}-t_i}
\begin{align}
    x_t = \frac{t_{i+1}-t}{t_{i+1}-t_i} x_{t_i} + \frac{t-t_{i}}{t_{i+1}-t_i} x_{t_{i+1}} + 
    \left(1- \left(\frac{t_{i+1}-t}{t_{i+1}-t_i}\right)^2 - \left(\frac{t-t_{i}}{t_{i+1}-t_i}\right)^2\right)\textsc{nnet}(t,x_{t_i},x_{t_{i+1}},\eta)\,.
    \nonumber
\end{align}
\normalsize
%For example, for a time-evolving system sampled discretely in time, we might enforce that our sampling distribution match the marginals $\mu_{t_i}$ given by the dataset.  
%Such examples are prevalent in trajectory inference problems in biological applications \citep{schiebinger2019optimal, tong2023conditional}.
%Introducing Lagrange multipliers for each intermediate marginal constraint in \cref{eq:general_lagr_min}, we obtain
% \RB{FIX ORDERING HERE?}
% \scriptsize
% \begin{align}%\label{eq:multi-marginal}
% \hspace{-.1cm} 
% %\cS_{\cL}&(\{\mu_{t_i}\}) = 
% \sup \limits_{\lagr_t, \lambda_{t_i}} \inf \limits_{\qm_t} ~ \int \lagr_1 \mu_1 dx_1 -  \int \lagr_0 \mu_0 dx_0 
% + \sum \limits_{i=1}^{M-2} \int  \lambda_{t_i} \big(  \mu_{t_i} - \qm_{t_i} \big)   dx_{t_i}  
% %\\
% %&\phantom{(\cL, \{\}=}
% -\int_0^1  \int  
% \left(\frac{\partial \lagr_t}{\partial t} + K^*[x_t,\lagr_t] + U[x_t,\lagr_t]
% %\hj[ \lagr_t, x_t] 
% \right)
%  \qm_t dx_t dt.  \nonumber
% \end{align}
% \normalsize

\vheader
\paragraph{Discontinuous Interpolation}
\vheader
The support of the optimal distribution path $\qm_t$ might be disconnected, as in \cref{fig:examples_a}.
Thus, it may be impossible to interpolate continuously between independent
%ly drawn 
samples from the marginals while staying in the support of the optimal path.
To allow for a discontinuous interpolation, we pass a discontinuous indicator variable $\mathbbm{1}[t < 0.5]$ to the model $\qm_t(x,\eta)$.
\vheader



==> text/app_sb.tex <==
%%%%%%%%%%%% \usepartialt includes extra term in Potential Energy, but simplifies final dual and allows for time-dependent SB %%%%%%%%%%%%%%%%
\def\usepartialt{1}
%\def\usepartialt{0}
\def\dummyfalse{0}
\section{Additional Examples}\label{app:additional_examples}
\subsection{Schrödinger Bridge}\label{app:sb}
To recover the Schrödinger Bridge problem, we proceed with a very particular choice of potential energy inspired by the \textit{generalized} Schrödinger Bridge problem in \citet{leger2021hopf}.   We essentially perform the derivations in their Sec. 2.3 in reverse to obtain a suitable potential energy.   

\textbf{Wasserstein-2 Gradient}
We begin by recalling the definintion of the Wasserstein gradient (\citet{figalli2021invitation} Sec. 4.2).  The Riemannian gradient of a functional $ \cF[\qm ] $ is the unique tangent vector such that the differential $d_{\dot{\qm}} \cF[\qm] $  in the direction $\dot{\qm}$ is given by the inner product $d_{\dot{\qm}} \cF[\qm ]  = \wmetricat{ \gradw \cF[\qm], \dot{\qm} }{\qm}$.  For the $W_2$ metric in \cref{eq:w2_metric}, we obtain the 
Wasserstein-2 gradient $ \gradw \cF[\qm ] \in T^{W_2}_{\qm} \wmanifold$ as
\begin{align}
    \gradw \cF[\qm ] = -\langle \nabla, \qm ~\nabla \frac{\delta \cF}{\delta \qm} \rangle .
\end{align}


\paragraph{Generalized Schrödinger Bridge}  \citet{leger2021hopf} consider a `generalized' \gls{SB} problem, where the dynamics include an additional drift corresponding to the gradient flow of a functional $\cF[\qm_t]$,
\begin{align}
\cS_{gSB}(\mu_{0,1}) = \inf \limits_{\qm_t, v_t}
%{(\qm_t, \dot{\qm}_t)} 
\int_0^1 
 \frac{1}{2} \| v_t \|^2 \qm_t dx_t
 %\frac{1}{2} \wmetricat{ \dot{\qm}_t, \dot{\qm}_t }{\qm_t} 
 \st \dot{\qm}_t &= -\langle \nabla, \qm_t \vel_t \rangle - \gradw \cF[\qm_t] \quad \qm_0 = \mu_0, \,\, \qm_1 = \mu_1 \label{eq:gsb} 
 %\\
% &=  -\langle \nabla, \qm_t \vel_t \rangle -\langle \nabla, \qm_t \nabla \frac{\delta \cF[\qm_t]}{\delta \qm_t}  \rangle 
\end{align}
which recovers \cref{eq:sb_std} in the main text for $\cF[\qm_t]$ equal to the negative Shannon entropy.

\begin{proposition}[\textbf{Dual Optimization and Potential Energy for Generalized Schrödinger Bridge}] Consider the Wasserstein-2 kinetic energy $\cK[\qm_t, \dot{\qm}_t] = \frac{1}{2} \wmetricat{ \dot{\qm}_t, \dot{\qm}_t }{\qm_t}$ and potential energy 
\ifx\usepartialt\dummyfalse
\begin{align}
    \cU[\qm_t, t] &=  -\lagrsbat{} \wnormat{ 
    \gradw \cF[\qm_t]
    %\nabla \frac{\delta \cF}{\delta \qm_t}
    }{\qm_t} \label{eq:potential_sb}
    \\
    \cU[\qm_1, 1] &=  -\sqrttwolagrsbat{} \int \frac{\delta \cF[\qm_1]}{\delta \qm_1} d\mu_1, \quad  \text{and} \quad \cU[\qm_0, 0] =  \sqrttwolagrsbat{}\int\frac{\delta \cF[\qm_0]}{\delta \qm_0} d\mu_0 ,
\end{align}
\else
\begin{align}
    \cU[\qm_t, t] &=  -\lagrsbat{t} \wnormat{ 
    \gradw \cF[\qm_t]
    %\nabla \frac{\delta \cF}{\delta \qm_t}
    }{\qm_t} 
     +  \int \frac{\partial }{\partial t}\left( \sqrttwolagrsbat{t} \frac{\delta \cF[\qm_t]}{\delta \qm_t}\right)~\qm_t~ dx_t, \quad \label{eq:potential_sb}
    \\
    \cU[\qm_1, 1] &=  -\sqrttwolagrsbat{1} \int \frac{\delta \cF[\qm_1]}{\delta \qm_1} d\mu_1, \quad \text{and} \quad \cU[\qm_0, 0] =  \sqrttwolagrsbat{0}\int\frac{\delta \cF[\qm_0]}{\delta \qm_0} d\mu_0 ,
\end{align}
for a Lagrangian optimization in the form of \cref{eq:general_lagr_min}.   In particular, the optimization $\cS_{gSB} = \inf_{\qm_t} \int_0^1 \cL[\qm_t, \dot{\qm}_t, t] dt = \inf_{\qm_t} \int_0^1 \cK[\qm_t, \dot{\qm}_t,t] -\cU[\qm_t, t] dt$ subject to marginal constraints $\qm_0 = \mu_0$ and $\qm_1 = \mu_1$ has the following dual form,
\small
\begin{align}
 &\cS_{gSB} = \sup \limits_{\Phi_t} \inf \limits_{\qm_t} ~ \int \Phi_1 d\mu_1 
  -  \int \Phi_0 d\mu_0   -\int_0^1 \int  \Bigg( \frac{\partial \Phi_t }{\partial t}  +\frac{1}{2} \big\| \nabla \Phi_t \big\|^2  - \sqrttwolagrsbat{t}  \big\langle \nabla \Phi_t, \nabla  \frac{\delta \cF[\qm_t]}{\delta \qm_t} \big\rangle 
\Bigg) \qm_t dx_t dt \label{eq:gsb_final}.
\end{align}
\normalsize
\end{proposition}
\textit{Remark:} We note that the $\int \frac{\partial }{\partial t}\left( \sqrttwolagrsbat{t} \frac{\delta \cF[\qm_t]}{\delta \qm_t}\right) \qm_t dx_t$ term in the potential energy is not necessary for the Schrödinger Bridge problem with time-independent diffusion coefficent, as presented in \cref{example:sb}.   See \cref{example:sb_app} below.
%\end{remark}
% We proceed with the Wasserstein-2 kinetic energy $\cK[\qm_t, \dot{\qm}_t] = \frac{1}{2} \wmetricat{ \dot{\qm}_t, \dot{\qm}_t }{\qm_t}$ and the potential energy
% \ifx\usepartialt\dummyfalse
% \begin{align}
%     \cU[\qm_t, t] &=  -\lagrsbat{} \wnormat{ 
%     \gradw \cF[\qm_t]
%     %\nabla \frac{\delta \cF}{\delta \qm_t}
%     }{\qm_t} \label{eq:potential_sb}
%     \\
%     \cU[\qm_1, 1] &=  -\sqrttwolagrsbat{} \int \frac{\delta \cF[\qm_1]}{\delta \qm_1} d\mu_1, \quad  \text{and} \quad \cU[\qm_0, 0] =  \sqrttwolagrsbat{}\int\frac{\delta \cF[\qm_0]}{\delta \qm_0} d\mu_0 .
% \end{align}
% \else
% \begin{align}
%     \cU[\qm_t, t] &=  -\lagrsbat{t} \wnormat{ 
%     \gradw \cF[\qm_t]
%     %\nabla \frac{\delta \cF}{\delta \qm_t}
%     }{\qm_t} 
%      +  \int \frac{\partial }{\partial t}\left( \sqrttwolagrsbat{t} \frac{\delta \cF[\qm_t]}{\delta \qm_t}\right)~\qm_t~ dx_t, \quad \label{eq:potential_sb}
%     \\
%     \cU[\qm_1, 1] &=  -\sqrttwolagrsbat{1} \int \frac{\delta \cF[\qm_1]}{\delta \qm_1} d\mu_1, \quad \text{and} \quad \cU[\qm_0, 0] =  \sqrttwolagrsbat{0}\int\frac{\delta \cF[\qm_0]}{\delta \qm_0} d\mu_0 .
% \end{align}
% where the $\frac{\partial }{\partial t}\left( \sqrttwolagrsbat{t} \frac{\delta \cF[\qm_t]}{\delta \qm_t}\right)$ is not necessary for the Schrödinger Bridge problem with time-independent diffusion coefficent presented in \cref{example:sb}.
%     \fi
\begin{proof}
With two endpoint marginal constraints and the $W_2$ tangent space parameterized by the continuity equation $\dot{\qm}_t = -\langle \nabla, \qm_t \vel_t \rangle$, the overall Lagrangian optimization, with $\cL[\qm_t, \dot{\qm}_t, t] = \cK[\qm_t, \dot{\qm}_t] -\cU[\qm_t, t]$, becomes
\ifx\usepartialt\dummyfalse
\begin{align}
%\begin{split}
\cS(\cL_{gSB}, \{\mu_{0,1}\}) &= \inf \limits_{\qm_t, \vel_t} \int_0^1 \int \left( \frac{1}{2}\big\| \vel_t \big\|^2  + \lagrsbat{} \big\| \nabla \frac{\delta \cF[\qm_t]}{\delta \qm_t} \big\|^2  \right) ~ \qm_t dx_t dt  \nonumber \\
&\phantom{\inf \limits_{(\qm_t, \dot{\qm}_t)} }  + \sqrttwolagrsbat{} \int \frac{\delta \cF[\qm_1]}{\delta \qm_1} d\mu_1 - \sqrttwolagrsbat{}\int\frac{\delta \cF[\qm_0]}{\delta \qm_0} d\mu_0 \label{eq:overall_sb}\\[1.25ex]
\quad \st &\quad \dot{\qm}_t  = -\langle \nabla, \qm_t \vel_t \rangle 
\qquad \qm_{0}   = \mu_{0}, \,\, \qm_1 = \mu_1 .\nonumber
%\end{split}
 \end{align}
\else
\begin{align}
%\begin{split}
\cS(\cL_{gSB}, \{\mu_{0,1}\}) &= \inf \limits_{\qm_t, \vel_t} \int_0^1 \int \left( \frac{1}{2}\big\| \vel_t \big\|^2  + \lagrsbat{} \big\| \nabla \frac{\delta \cF[\qm_t]}{\delta \qm_t} \big\|^2   - \sqrttwolagrsbat{t} \frac{\partial }{\partial t}\left(\frac{\delta \cF[\qm_t]}{\delta \qm_t}\right) \right) ~ \qm_t dx_t dt  \nonumber \\
&\phantom{\inf \limits_{(\qm_t, \dot{\qm}_t)} }  + \sqrttwolagrsbat{t} \int \frac{\delta \cF[\qm_1]}{\delta \qm_1} d\mu_1 - \sqrttwolagrsbat{t}\int\frac{\delta \cF[\qm_0]}{\delta \qm_0} d\mu_0 \label{eq:overall_sb}\\[1.25ex]
\quad \st &\quad \dot{\qm}_t  = -\langle \nabla, \qm_t \vel_t \rangle 
\qquad \qm_{0}   = \mu_{0}, \,\, \qm_1 = \mu_1 .\nonumber
%\end{split}
\end{align}
\fi
Introducing Lagrange multipliers $\lagr_t$ and eliminating $\vel_t$, we obtain 
\ifx\usepartialt\dummyfalse
\begin{align}
\cS_{gSB} &= \sup \limits_{\lagr_t} \inf \limits_{\qm_t} ~ \int \lagr_1 d\mu_1 -  \int \lagr_0 d\mu_0  + \sqrttwolagrsbat{} \int \frac{\delta \cF[\qm_1]}{\delta \qm_1} d\mu_1 - \sqrttwolagrsbat{}\int\frac{\delta \cF[\qm_0]}{\delta \qm_0} d\mu_0 \label{eq:gsb0}
 \\
&\phantom{(\cL, \{\}=}-\int_0^1 \int  \left( \frac{\partial \lagr_t }{\partial t}  + \frac{1}{2}   \big\|\nabla \lagr_t\big\|^2  -  \lagrsbat{} \big\| \nabla \frac{\delta \cF[\qm_t]}{\delta \qm_t}\big\|^2 
%- \sqrttwolagrsbat{} \frac{\partial }{\partial t}\left(\frac{\delta \cF[\qm_t]}{\delta \qm_t}
\right) \qm_t dx_t dt \nonumber 
\end{align}
\else
\begin{align}
\cS_{gSB} &= \sup \limits_{\lagr_t} \inf \limits_{\qm_t} ~ \int \lagr_1 d\mu_1 -  \int \lagr_0 d\mu_0  + \sqrttwolagrsbat{1} \int \frac{\delta \cF[\qm_1]}{\delta \qm_1} d\mu_1 - \sqrttwolagrsbat{0}\int\frac{\delta \cF[\qm_0]}{\delta \qm_0} d\mu_0 \label{eq:gsb0}
 \\
&\phantom{(\cL, \{\}=}-\int_0^1 \int  \left( \frac{\partial \lagr_t }{\partial t}  + \frac{1}{2}   \big\|\nabla \lagr_t\big\|^2  -\lagrsbat{t} \big\| \nabla \frac{\delta \cF[\qm_t]}{\delta \qm_t}\big\|^2 
+  \frac{\partial }{\partial t}\left(\sqrttwolagrsbat{t}\frac{\delta \cF[\qm_t]}{\delta \qm_t}
\right) \right) \qm_t dx_t dt \nonumber 
\end{align}
\fi



\textit{Fokker-Planck Reparameterization:} %\RB{Fokker-Planck Reparametrization}
We consider the following reparameterization, 
\ifx\usepartialt\dummyfalse
\begin{align}
     \lagr_t = \Phi_t - \sqrttwolagrsbat{}  \frac{\delta \cF[\qm_t]}{\delta \qm_t}, \qquad \qquad \nabla \lagr_t  =  \nabla \Phi_t- \sqrttwolagrsbat{} \nabla \frac{\delta \cF[\qm_t]}{\delta \qm_t} . \label{eq:reparam}
\end{align}
In the case of the standard \textsc{sb} problem with $\cF[\qm_t] = -H[\qm_t]$, we have $\nabla \frac{\delta \cF[\qm_t]}{\delta \qm_t} = \nabla \log \qm_t$.   Recalling that our action function $\lagr_t$ arose from enforcing the continuity equation, we can interpret $\nabla \lagr_t =  \nabla \Phi_t - \sqrttwolagrsbat{} \nabla \log  \qm_t $ as the drift of the \textit{probability flow \textsc{ode}}.   Substituting into the continuity equation $\dot{\qm}_t = -\langle \nabla, \qm_t \nabla \lagr_t \rangle$ and simplifying, we see that $\nabla \Phi_t $ corresponds to the drift in the Fokker Planck equation $\dot{\qm}_t =  -\langle \nabla, \qm_t \nabla \Phi_t \rangle - \sqrttwolagrsbat{} \langle \nabla, \qm_t \nabla \log \qm_t \rangle = -\langle \nabla, \qm_t \nabla \Phi_t \rangle + \sqrttwolagrsbat{} \Delta \qm_t$.  

More generally, \citet{leger2021hopf} consider dynamics of the form $\dot{\qm}_t =  -\langle \nabla, \qm_t \nabla \Phi_t \rangle - \sqrttwolagrsbat{} \gradw \cF[\qm_t] = \dot{\qm}_t =  -\langle \nabla, \qm_t \nabla \Phi_t \rangle + \sqrttwolagrsbat{} \langle \nabla, \qm_t \nabla \frac{\delta  \cF[\qm_t]}{\delta \qm_t} \rangle $.
See \cref{eq:fp_lagr}  below.

\else
\begin{align}
     \lagr_t = \Phi_t - \sqrttwolagrsbat{t}  \frac{\delta \cF[\qm_t]}{\delta \qm_t}, \qquad \qquad \nabla \lagr_t  =  \nabla \Phi_t- \sqrttwolagrsbat{t} \nabla \frac{\delta \cF[\qm_t]}{\delta \qm_t} . \label{eq:reparam}
\end{align}
In the case of the standard \textsc{sb} problem with $\cF[\qm_t] = -H[\qm_t]$, we have $\nabla \frac{\delta \cF[\qm_t]}{\delta \qm_t} = \nabla \log \qm_t$ (see \cref{example:sb_app} below).   Recalling that our action function $\lagr_t$ arose from enforcing the continuity equation, we can interpret $\nabla \lagr_t =  \nabla \Phi_t - \sqrttwolagrsbat{t} \nabla \log  \qm_t $ as the drift of the \textit{probability flow \textsc{ode}}.   Substituting into the continuity equation $\dot{\qm}_t = -\langle \nabla, \qm_t \nabla \lagr_t \rangle$ and simplifying, we see that $\nabla \Phi_t $ corresponds to the drift in the Fokker Planck equation $\dot{\qm}_t =  -\langle \nabla, \qm_t \nabla \Phi_t \rangle - \sqrttwolagrsbat{t} \langle \nabla, \qm_t \nabla \log \qm_t \rangle = -\langle \nabla, \qm_t \nabla \Phi_t \rangle + \sqrttwolagrsbat{t} \Delta \qm_t$.  

More generally, \citet{leger2021hopf} consider dynamics of the form $\dot{\qm}_t =  -\langle \nabla, \qm_t \nabla \Phi_t \rangle - \sqrttwolagrsbat{t} \gradw \cF[\qm_t] = \dot{\qm}_t =  -\langle \nabla, \qm_t \nabla \Phi_t \rangle + \sqrttwolagrsbat{t} \langle \nabla, \qm_t \nabla \frac{\delta  \cF[\qm_t]}{\delta \qm_t} \rangle $.   See \cref{eq:fp_lagr}  below.
\fi


\ifx\usepartialt\dummyfalse
\textit{Dual Objective:} Substituting \cref{eq:reparam} into \cref{eq:gsb0},
\begin{align}
 \hspace*{-.2cm}\cS_{gSB}& = \sup \limits_{\Phi_t} \inf \limits_{\qm_t} \int \Phi_1 d\mu_1 \pm 
 \cancel{ \sqrttwolagrsbat{}  \int  \frac{\delta \cF[\qm_1]}{\delta \qm_1} d\mu_1 } -  \int \Phi_0 d\mu_0 \pm \cancel{ \sqrttwolagrsbat{} \int  \frac{\delta \cF[\qm_0]}{\delta \qm_0} d\mu_0} \\
-&\int_0^1 \int  \Bigg( \frac{\partial \Phi_t }{\partial t}  - \sqrttwolagrsbat{} \frac{\partial }{\partial t}\left(   \frac{\delta \cF[\qm_t]}{\delta \qm_t} \right)  +\frac{1}{2} \left\| \nabla \Phi_t - \sqrttwolagrsbat{} \nabla  \frac{\delta \cF[\qm_t]}{\delta \qm_t}\right\|^2 -
\lagrsbat{} \left\| \nabla \frac{\delta \cF[\qm_t]}{\delta \qm_t}\right\|^2
\Bigg) \qm_t ~ dx_t dt \nonumber 
\end{align}
Expanding the inner product term, we see that the Wasserstein gradient norm terms cancel, leaving
\begin{align}
 \cS_{gSB} = \sup \limits_{\Phi_t} \inf \limits_{\qm_t}  \int \Phi_1 d\mu_1 
  -  \int \Phi_0 d\mu_0   
-\int_0^1 \int  \Bigg( &\frac{\partial \Phi_t }{\partial t} - \sqrttwolagrsbat{} \frac{\partial }{\partial t}\left(   \frac{\delta \cF[\qm_t]}{\delta \qm_t} \right) \\
&+\frac{1}{2} \big\| \nabla \Phi_t \big\|^2  - \sqrttwolagrsbat{}  \big\langle \nabla \Phi_t, \nabla  \frac{\delta \cF[\qm_t]}{\delta \qm_t} \big\rangle 
\Bigg) \qm_t dx_t dt \nonumber
\end{align}
\else 
\textit{Dual Objective:} Substituting \cref{eq:reparam} into \cref{eq:gsb0},
\begin{align}
 \cS_{gSB} = \sup \limits_{\Phi_t} \inf \limits_{\qm_t} &\int \Phi_1 d\mu_1 \pm 
 \cancel{ \sqrttwolagrsbat{1}  \int  \frac{\delta \cF[\qm_1]}{\delta \qm_1} d\mu_1 } -  \int \Phi_0 d\mu_0 \pm \cancel{ \sqrttwolagrsbat{0} \int  \frac{\delta \cF[\qm_0]}{\delta \qm_0} d\mu_0} \\
-&\int_0^1 \int  \Bigg( \frac{\partial \Phi_t }{\partial t}  - \cancel{\frac{\partial }{\partial t}\left(\sqrttwolagrsbat{t}    \frac{\delta \cF[\qm_t]}{\delta \qm_t} \right) } + \cancel{\frac{\partial }{\partial t}\left(  \sqrttwolagrsbat{t}  \frac{\delta \cF[\qm_t]}{\delta \qm_t} \right) } \nonumber \\
& \phantom{\int_0^1 } +\frac{1}{2} \left\langle \nabla \Phi_t - \sqrttwolagrsbat{t} \nabla  \frac{\delta \cF[\qm_t]}{\delta \qm_t}, \nabla \Phi_t - \sqrttwolagrsbat{t} \nabla  \frac{\delta \cF[\qm_t]}{\delta \qm_t} \right\rangle -
\lagrsbat{t} \left\| \nabla \frac{\delta \cF[\qm_t]}{\delta \qm_t}\right\|^2
\Bigg) \qm_t ~ dx_t dt \nonumber 
\end{align}
Expanding the inner product term, we see that the Wasserstein gradient norm terms cancel, leaving
\begin{align}
 &\cS_{gSB} = \sup \limits_{\Phi_t} \inf \limits_{\qm_t} ~ \int \Phi_1 d\mu_1 
  -  \int \Phi_0 d\mu_0   -\int_0^1 \int  \Bigg( \frac{\partial \Phi_t }{\partial t}  +\frac{1}{2} \big\| \nabla \Phi_t \big\|^2  - \sqrttwolagrsbat{t}  \big\langle \nabla \Phi_t, \nabla  \frac{\delta \cF[\qm_t]}{\delta \qm_t} \big\rangle 
\Bigg) \qm_t dx_t dt %\label{eq:gsb_final}
\end{align}
\fi
which completes the proof.
\end{proof}


\paragraph{Lagrangian in the Fokker-Planck Reparameterization}
To justify the connection with the (generalized) Schrödinger Bridge problem,  we associate the dual in \cref{eq:gsb_final} to a Lagrangian optimization with Fokker-Planck style dynamics   %Integrating by parts in $t$ and $x$,
% \begin{align*}
%  \cS_{gSB} &= \sup \limits_{\Phi_t} \inf \limits_{\qm_t} ~ \int \Phi_1 d\mu_1 
%   -  \int \Phi_0 d\mu_0   -\int_0^1 \int  \Bigg( \frac{\partial \Phi_t }{\partial t}  +\frac{1}{2} \big\| \nabla \Phi_t \big\|^2  - \sqrttwolagrsbat{t}  \big\langle \nabla \Phi_t, \nabla  \frac{\delta \cF[\qm_t]}{\delta \qm_t} \big\rangle 
% \Bigg) \qm_t dx_t dt \\
% &=\sup \limits_{\Phi_t} \inf \limits_{\qm_t} ~ \int \Phi_1 (d\mu_1 - d\qm_1)
%   -  \int \Phi_0 (d\mu_0 - d\qm_0)  + \int_0^1 \int  \frac{\partial \qm_t}{\partial t} \Phi_t dx_t dt \\
% &\phantom{\sup \limits_{\Phi_t} \inf \limits_{\qm_t} } + \int_0^1 \int  \Bigg( \frac{1}{2} \big\| \nabla \Phi_t \big\|^2  - \sqrttwolagrsbat{t}  \big\langle \nabla \Phi_t, \nabla  \frac{\delta \cF[\qm_t]}{\delta \qm_t} \big\rangle 
% \Bigg) \qm_t dx_t dt
% \end{align*}
\begin{align}
 \hspace*{-.2cm} \cS_{gSB}(\mu_{0,1}) = \inf \limits_{(\qm_t, \dot{\qm}_t)} \int_0^1 \int \frac{1}{2} \| \vel_t \|^2 \qm_t dx_t dt \st  \dot{\qm}_t &= - \langle \nabla, \qm_t \vel_t \rangle 
 %- \gradw \cF[\qm_t], 
 + \langle \nabla, \qm_t \nabla \frac{\delta \cF[\qm_t]}{\delta \qm_t} \rangle, 
 \label{eq:fp_lagr}\\
 \qm_0 &= \mu_0, \,\, \qm_1 = \mu_1 . \nonumber
\end{align}
To show this, we perform similar derivations as in \cref{app:dual_kinetic} in reverse:  introducing a Lagrange multipler $\Phi_t$ to enforce the constraints, integrating by parts in $t$ and $x$, and eliminating $\vel_t = \nabla \Phi_t$.  

Note that the dynamics can be written using the $W_2$ gradient of $\cF[\qm_t]$, as $\dot{\qm}_t = - \langle \nabla, \qm_t \vel_t \rangle - \gradw \cF[\qm_t] $ as in \citet{leger2021hopf}, while the formulation in \cref{eq:fp_lagr} matches well-known optimal control formulations of the Schrödinger Bridge problem \citep{chen2016relation, chen2021stochastic}.



\begin{example}[\textbf{Schrödinger Bridge with Time-Dependent Diffusion Coefficient}]\label{example:sb_app}
Choosing $\cF[\qm_t] = -H[\qm_t]$, we have $\nabla \frac{\delta \cF[\qm_t]}{\delta \qm_t} = \nabla \log \qm_t$. 
Simplifying and integrating by parts, the final term in \cref{eq:gsb_final} becomes
\begin{align}
\int_0^1 \int  \big\langle \nabla \Phi_t, \nabla \log \qm_t \big\rangle 
 \qm_t dx_t dt = \int_0^1 \int  \big\langle \nabla \Phi_t, \nabla \qm_t \big\rangle 
 dx_t dt = - \int_0^1 \int \left( \Delta \Phi_t \right) ~ \qm_t~ dx_t dt 
\end{align}
which yields the eventual dual objective
\begin{align}
 \hspace*{-.2cm} \cS_{SB} = \sup \limits_{\Phi_t} \inf \limits_{\qm_t} ~ \int \Phi_1 d\mu_1 
  -  \int \Phi_0 d\mu_0   -\int_0^1 \int  \Bigg( \frac{\partial \Phi_t }{\partial t}  +\frac{1}{2} \big\| \nabla \Phi_t \big\|^2  + \sqrttwolagrsbat{t}  \Delta \Phi_t
\Bigg) \qm_t dx_t dt \label{appeq:sb_t_final}.
\end{align}
\end{example}

%\subsubsection{Schrödinger Bridge Examples}
\begin{example}[\textbf{Schrödinger Bridge with Time-Independent Diffusion Coefficient}]
When $\sqrttwolagrsbat{}$ is independent of $t$, the additional term $\int \frac{\partial }{\partial t}\left( \sqrttwolagrsbat{} \frac{\delta \cF[\qm_t]}{\delta \qm_t}\right)~\qm_t~ dx_t$ in the potential energy \cref{eq:potential_sb} vanishes for the entropy functional, with $\frac{\delta \cF[\qm_t]}{\delta \qm_t} = \log \qm_t$ and
\begin{align}
\int \frac{\partial }{\partial t}\left( \sqrttwolagrsbat{} \frac{\delta \cF[\qm_t]}{\delta \qm_t}\right)~\qm_t~ dx_t = \sqrttwolagrsbat{} \int   \frac{\partial \log \qm_t}{\partial t}~\qm_t~ dx_t = \sqrttwolagrsbat{} \frac{\partial }{\partial t} \int    \qm_t~ dx_t = 0 .
\end{align}
Note that this observation simplifies the potential energy and derivations above, but preserves the same dual objective from \cref{appeq:sb_t_final}.
\end{example}

\begin{example}[Porous Medium Dynamics]\label{example:porous}
Consider the (scaled) negative Tsallis entropy $\cF[\qm_t] = -H_\alpha[\qm_t] =  \frac{1}{q(q-1)} \int \qm_t^{q} dx_t$.   In this case, we have
\begin{align}
\frac{\delta \cF[\qm_t]}{\delta \qm_t} = \frac{1}{q-1} \qm_t(x_t)^{q-1} \qquad \qquad \nabla \frac{\delta \cF[\qm_t]}{\delta \qm_t} =  \qm_t(x_t)^{q-2}  \nabla \qm_t(x_t)
\end{align}
Reparameterizing the continuity equation with \cref{eq:reparam} yields a non-linear Fokker-Planck equation with $q$-Brownian motion, after simplifying $\langle \nabla, \qm_t \qm_t^{q-2}  \nabla \qm_t \rangle = \langle \nabla,  \qm_t^{q-1}  \nabla \qm_t \rangle = \langle \nabla, \frac{1}{q}\nabla \qm_t^{q}\rangle = \frac{1}{q}\Delta \qm_t^q$,
\begin{align}
 \text{For} \,\, \nabla \lagr_t  =  \nabla \Phi_t- \sqrttwolagrsbat{t} \qm_t^{q-2} \nabla \qm_t , \quad \text{and} \quad\dot{\qm}_t &= -\langle \nabla, \qm_t \nabla \phi_t \rangle \qquad  \nonumber \\
 \implies \quad \dot{\qm}_t &= -\langle \nabla, \qm_t \nabla \Phi_t \rangle + \sqrttwolagrsbat{t} \langle \nabla, \qm_t \qm_t^{q-2}  \nabla \qm_t \rangle  \nonumber \\
 \implies \quad \dot{\qm}_t &= -\langle \nabla, \qm_t \nabla \Phi_t \rangle + \sqrttwolagrsbat{t} \frac{1}{q}\Delta \qm_t^q.
\end{align}
For the appropriate potential energy in \cref{eq:potential_sb}, we apply similar simplifications to the final term in \cref{eq:gsb_final}
\begin{align}
  \int_0^1 \int \sqrttwolagrsbat{t}  \big\langle \nabla \Phi_t, \qm_t^{q-2}  \nabla \qm_t  \big\rangle 
 \qm_t dx_t dt 
 &= \int_0^1 \int \sqrttwolagrsbat{t}  \big\langle \nabla \Phi_t, \frac{1}{q} \nabla \qm_t^q \big\rangle  dx_t dt
 = - \int_0^1 \int \sqrttwolagrsbat{t}  \frac{1}{q} ( \Delta \Phi_t ) \qm_t^q  dx_t dt \nonumber
\end{align}
Substituting back into \cref{eq:gsb_final}, 
\begin{align}
 \cS_{PM} = \sup \limits_{\Phi_t} \inf \limits_{\qm_t} ~ \int \Phi_1 d\mu_1 
  -  \int \Phi_0 d\mu_0   -\int_0^1 \int  \Bigg( \frac{\partial \Phi_t }{\partial t}  +\frac{1}{2} \big\| \nabla \Phi_t \big\|^2  + \sqrttwolagrsbat{t} \frac{1}{q} ( \Delta \Phi_t ) \qm_t^{q-1}  
\Bigg) \qm_t dx_t dt \nonumber
%\label{eq:gsb_final}
\end{align}
In contrast to the case of $q=1$, we have a nonlinear term in the density $\qm_t^{q-1}$, which cannot be optimized simply by drawing samples from $\qm_t$ and thus is not immediately tractable under our proposed framework.
\end{example}












==> text/app_sb_redo.tex <==

\subsection{Schrödinger Bridge}\label{app:sb}
%To recover the Schrödinger Bridge problem, we proceed with a particular choice of potential energy inspired by the \textit{generalized} Schrödinger Bridge problem in \citet{leger2021hopf}.  % We essentially perform the derivations in their Sec. 2.3 in reverse to obtain a suitable potential energy.
In this section, we derive potential energies and tractable objectives corresponding to the Schrödinger Bridge problem 
\begin{align}
\hspace*{-.2cm} cS_{SB}(\{\mu_{0,1}\}) = \inf \limits_{\qm_t, v_t}
%{(\qm_t, \dot{\qm}_t)} 
\int_0^1 
 \frac{1}{2} \| v_t \|^2 \qm_t dx_t
 %\frac{1}{2} \wmetricat{ \dot{\qm}_t, \dot{\qm}_t }{\qm_t} 
 \st \dot{\qm}_t &= -\langle \nabla, \qm_t \vel_t \rangle - \sqrttwolagrsbat{} \Delta \qm_t
 \quad \qm_0 = \mu_0, \,\, \qm_1 = \mu_1 . \label{eq:fp_sb} 
 %\\
% &=  -\langle \nabla, \qm_t \nabla \action_t \rangle -\langle \nabla, \qm_t \nabla \frac{\delta \cF[\qm_t]}{\delta \qm_t}  \rangle 
\end{align}
which we will solve using the following (linear in $\qm_t$) dual objective from \cref{eq:sb_t_final} (see \cref{example:sb_app})
\small
\begin{align}
 \hspace*{-.2cm} \cS_{SB}(\{\mu_{0,1}\}) = \sup \limits_{\Phi_t} \inf \limits_{\qm_t} ~ \int \Phi_1 \mu_1 dx_1 
  -  \int \Phi_0 \mu_0 dx_0   -\int_0^1 \int  \Bigg( \frac{\partial \Phi_t }{\partial t}  +\frac{1}{2} \big\| \nabla \Phi_t \big\|^2  + \sqrttwolagrsbat{t}  \Delta \Phi_t
\Bigg) \qm_t dx_t dt .\nonumber
\end{align}
\normalsize
We first present background on $W_2$ gradients and the generalized \gls{SB} problem from \citet{leger2021hopf}.
%In \cref{prop:sb} below, we pose a Wasserstein Lagrangian flow and derive its dual objective, before showing its equivalence with the generalized \gls{SB} problem in \cref{eq:fp_sb}. %in \cref{prop:sb}.

%frame the problem in \cref{eq:fp_sb} as a Wasserstein Lagrangian flow, before showing the equivalence of \cref{eq:fp_sb}


\textbf{Wasserstein-2 Gradient}
We begin by recalling the definintion of the Wasserstein gradient (\citet{figalli2021invitation} Sec. 4.2).  The Riemannian gradient of a functional $ \cF[\qm ] $ is the unique tangent vector such that the differential $d_{\dot{\qm}} \cF[\qm] $  in the direction $\dot{\qm}$ is given by the inner product $d_{\dot{\qm}} \cF[\qm ]  = \wmetricat{ \gradw \cF[\qm], \dot{\qm} }{\qm}$.  For the $W_2$ metric in \cref{eq:w2_metric}, we obtain the 
Wasserstein-2 gradient $ \gradw \cF[\qm ] \in T^{W_2}_{\qm} \wmanifold$ as
\begin{align}
    \gradw \cF[\qm ] = -\langle \nabla, \qm ~\nabla \frac{\delta \cF}{\delta \qm} \rangle.
\end{align}

\textbf{Generalized SB}
Slightly more generally than \cref{eq:fp_sb}, we consider the  `generalized' Schrödinger Bridge problem  in \citet{leger2021hopf}, which perturbs the standard continuity equation with an additional drift given by the Wasserstein-2 gradient of a functional $\cF[\qm_t]$
%\small
\begin{align}
\cS_{gSB}(\{\mu_{0,1}\}) = \inf \limits_{\qm_t, v_t}
%{(\qm_t, \dot{\qm}_t)} 
\int_0^1 
 \frac{1}{2} \| v_t \|^2 \qm_t dx_t
 %\frac{1}{2} \wmetricat{ \dot{\qm}_t, \dot{\qm}_t }{\qm_t} 
 \st \dot{\qm}_t &= -\langle \nabla, \qm_t \vel_t \rangle - \sqrttwolagrsbat{t} \gradw \cF[\qm_t], \,\, \qm_0 = \mu_0, \,\, \qm_1 = \mu_1  \label{eq:gsb}
 %\\ &= -\langle \nabla, \qm_t \vel_t \rangle + \sqrttwolagrsbat{t} \langle \nabla, \qm ~\nabla \frac{\delta \cF}{\delta \qm} \rangle    
 %\\
% &=  -\langle \nabla, \qm_t \nabla \action_t \rangle -\langle \nabla, \qm_t \nabla \frac{\delta \cF[\qm_t]}{\delta \qm_t}  \rangle 
\end{align}
\normalsize
where $\dot{\qm}_t = -\langle \nabla, \qm_t \vel_t \rangle - \sqrttwolagrsbat{t} \gradw \cF[\qm_t] = -\langle \nabla, \qm_t \vel_t \rangle + \sqrttwolagrsbat{t} \langle \nabla, \qm ~\nabla \frac{\delta \cF}{\delta \qm} \rangle$.
\cref{eq:gsb} recovers \cref{eq:sb_std} or \cref{eq:fp_sb} for $\cF[\qm_t]$ equal to the negative Shannon entropy.

\subsubsection{Dual Objectives for Generalized Schrödinger Bridge}
We proceed in two steps for cases related to the generalized \gls{SB} problem.   We begin by defining a Wasserstein-Lagrangian flow and deriving its Hamiltonian and dual objective and \cref{lemma:sb}.  We then perform a reparameterization corresponding to Fokker-Planck dynamics and the Hopf-Cole transform in \cref{prop:sb}, and show that the solution to the dual optimization corresponds to the solution to both our Lagrangain flow and the generalized \gls{SB} problem in \cref{eq:gsb}.

\begin{lemma}\label{lemma:sb}
Consider a Lagrangian defined using
\begin{align}
 \cK[\qm_t, \dot{\qm}_t, t] = \frac{1}{2} \wmetricat{ \dot{\qm}_t, \dot{\qm}_t }{\qm_t} \qquad \cU[\qm_t, t] &=  -\lagrsbat{t} \wnormat{ 
    \gradw \cF[\qm_t]
    }{\qm_t} 
     +  \int \frac{\partial }{\partial t}\left(\sqrttwolagrsbat{t} \frac{\delta \cF[\qm_t]}{\delta \qm_t}\right) ~\qm_t~ dx_t, \quad \nonumber % \\
     %&= - \lagrsbat{t}  
      % \int \|  \nabla \frac{\delta \cF[\qm_t]}{\delta \qm_t} \|^2 \qm_t dx_t +  \int \frac{\partial }{\partial t}\left(\sqrttwolagrsbat{t} \frac{\delta \cF[\qm_t]}{\delta \qm_t}\right) ~\qm_t~ dx_t, \nonumber
% \cL[\qm_t, \dot{\qm}_t, t] =  \frac{1}{2} \wmetricat{ \dot{\qm}_t, \dot{\qm}_t }{\qm_t} - \left( -\lagrsbat{t} \wnormat{ 
%     \gradw \cF[\qm_t]}{\qm_t} +  \int \frac{\partial }{\partial t}\left(\sqrttwolagrsbat{t} \frac{\delta \cF[\qm_t]}{\delta \qm_t}\right) ~\qm_t~ dx_t \right).
\end{align}
where $\wnormat{ 
    \gradw \cF[\qm_t]
    }{\qm_t} = \int \|  \nabla \frac{\delta \cF[\qm_t]}{\delta \qm_t} \|^2 \qm_t dx_t$.
The Hamiltonian is given by
\begin{align}
\cH[\qm_t, \lagr_t, t] =  \frac{1}{2}\int \| \nabla \lagr_t  \|^2 \qm_t dx_t -\lagrsbat{t}  
       \int \|  \nabla \frac{\delta \cF[\qm_t]}{\delta \qm_t} \|^2 \qm_t dx_t 
     + \int \frac{\partial }{\partial t}\left(\sqrttwolagrsbat{t} \frac{\delta \cF[\qm_t]}{\delta \qm_t}\right) \qm_t dx_t \label{eq:gsb_hamiltonian0}.
\end{align}
\normalsize
\end{lemma}
\paragraph{Remark:} We note that the $\int \frac{\partial }{\partial t}\left(\sqrttwolagrsbat{t} \frac{\delta \cF[\qm_t]}{\delta \qm_t}\right)  \qm_t dx_t$ term in the potential energy vanishes with time-independent diffusion coefficent, as presented in \cref{example:sb} (see \cref{example:sb_app} below). %is not necessary for the classical Schrödinger Bridge problem


\begin{proof}
The full Lagrangian in \cref{lemma:sb} is
\begin{align}
\cL[\qm_t, \dot{\qm}_t, t] =  \frac{1}{2} \wmetricat{ \dot{\qm}_t, \dot{\qm}_t }{\qm_t} - \left( -\lagrsbat{t} \int \|  \nabla \frac{\delta \cF[\qm_t]}{\delta \qm_t} \|^2 \qm_t dx_t    +  \int \frac{\partial }{\partial t}\left(\sqrttwolagrsbat{t} \frac{\delta \cF[\qm_t]}{\delta \qm_t}\right) ~\qm_t~ dx_t \right).
\end{align}
We now solve for the Hamiltonian, where we parametrize the tangent space using the continuity equation $\dot{\qm}_t = -\langle \nabla, \qm_t v_t\rangle$ and vector field $v_t$.  As in \cref{eq:from_continuity}-(\ref{eq:to_continuity}),
\footnotesize
\begin{align}
\cH[&\qm_t, \lagr_t, t] =  \sup_{\dot{\qm}_t} \int \dot{\qm}_t \lagr_t dx_t - \cL[\qm_t, \dot{\qm}_t,t] \label{eq:hamil_sb} \\
&= \sup_{v_t} \int  - \lagr_t \langle \nabla, \qm_t v_t \rangle dx_t - \frac{1}{2}\int \|  v_t \|^2 \qm_t dx_t -\lagrsbat{t}  
       \int \|  \nabla \frac{\delta \cF[\qm_t]}{\delta \qm_t} \|^2 \qm_t dx_t 
     + \int \frac{\partial }{\partial t}\left(\sqrttwolagrsbat{t} \frac{\delta \cF[\qm_t]}{\delta \qm_t}\right) \qm_t dx_t \nonumber \\
&=\sup \limits_{v_t} ~  \int  \langle \nabla \lagr_t,  v_t \rangle \qm_t   dx_t - \frac{1}{2}\int \|  v_t \|^2 \qm_t dx_t -\lagrsbat{t}  
       \int \|  \nabla \frac{\delta \cF[\qm_t]}{\delta \qm_t} \|^2 \qm_t dx_t 
     + \int \frac{\partial }{\partial t}\left(\sqrttwolagrsbat{t} \frac{\delta \cF[\qm_t]}{\delta \qm_t}\right) \qm_t dx_t \nonumber
%=\sup \limits_{v_t} ~  \int  \langle \nabla \lagr_t,  v_t \rangle \qm_t  ~ dx_t - \cK[\qm_t, \dot{\qm}_t,t] + \cU[\qm_t, t] .
\end{align}
\normalsize
which implies $v_t = \nabla \lagr_t $ as before.  Substituting into the above, we have 
\begin{align}
\cH[\qm_t, \lagr_t, t] =  \frac{1}{2}\int \| \nabla \lagr_t  \|^2 \qm_t dx_t -\lagrsbat{t}  
       \int \|  \nabla \frac{\delta \cF[\qm_t]}{\delta \qm_t} \|^2 \qm_t dx_t 
     + \int \frac{\partial }{\partial t}\left(\sqrttwolagrsbat{t} \frac{\delta \cF[\qm_t]}{\delta \qm_t}\right) \qm_t dx_t . \label{eq:gsb_hamiltonian}
\end{align}
which is of the form $\cH[\qm_t, \lagr_t, t]= \cK^*[\qm_t, \lagr_t, t] + \cU[\qm_t, t]$ and matches \citet{leger2021hopf} Eq. 8 up to the additional $\frac{\partial }{\partial t}\sqrttwolagrsbat{t}\frac{\delta \cF[\qm_t]}{\delta \qm_t}$ term, which will be used below to account for time-dependent $\sigma_t$.  
\end{proof}
% % Consider the Lagrangian
% % %Wasserstein Lagrangian Flow (\cref{eq:general_lagr_min}) with 
% % \begin{align}
% %  \cK[\qm_t, \dot{\qm}_t, t] = \frac{1}{2} \wmetricat{ \dot{\qm}_t, \dot{\qm}_t }{\qm_t} \qquad \cU[\qm_t, t] &=  -\lagrsbat{t} \wnormat{ 
% %     \gradw \cF[\qm_t]
% %     }{\qm_t} 
% %      +  \int \frac{\partial }{\partial t}\left(\sqrttwolagrsbat{t} \frac{\delta \cF[\qm_t]}{\delta \qm_t}\right) ~\qm_t~ dx_t, \quad \nonumber  \\
% %      &= - \lagrsbat{t}  
% %        \int \|  \nabla \frac{\delta \cF[\qm_t]}{\delta \qm_t} \|^2 \qm_t dx_t +  \int \frac{\partial }{\partial t}\left(\sqrttwolagrsbat{t} \frac{\delta \cF[\qm_t]}{\delta \qm_t}\right) ~\qm_t~ dx_t, \nonumber
% % % \cL[\qm_t, \dot{\qm}_t, t] =  \frac{1}{2} \wmetricat{ \dot{\qm}_t, \dot{\qm}_t }{\qm_t} - \left( -\lagrsbat{t} \wnormat{ 
% % %     \gradw \cF[\qm_t]}{\qm_t} +  \int \frac{\partial }{\partial t}\left(\sqrttwolagrsbat{t} \frac{\delta \cF[\qm_t]}{\delta \qm_t}\right) ~\qm_t~ dx_t \right).
% % \end{align}
% % The objective to the Wasserstein Lagrangian Flow 
% % \begin{align}\label{eq:general_lagr_min}
% % \cS_{\cL}(\{\mu_{0,1}\}) = \inf
% % \limits_{\qm_t}
% % %\limits_{(\qm_t, \dot{\qm}_t)} 
% % \int_0^1 \mathcal{L}[\qm_t, \dot{\qm}_t,t]dt 
% % %\,\, \text{s.t. } \,\, &\dot{\qm}_t = - \langle \nabla, \qm_t \vel_t \rangle + \qm_t \action_t, \, 
% % %\\ \text{ and } \,\,  
% % \quad \st \quad
% % \qm_0 = \mu_0, \qquad \qm_1 = \mu_1
% % %\qm_{t_i}   = \mu_{t_i} \quad (\forall \,\, 0\leq i \leq M-1).
% % \end{align}
% % matches the solution to the generalized \gls{SB} problem

% % The optimal solution $(\qm_t, \vel_t) = (\qm_t, \nabla \Phi_t)$
% % dual optimization
% % \begin{align}
% % \cS_\cL(\{\mu_{0,1}\}) &=  \inf \limits_{\qm_t} \sup \limits_{\Phi_t}  \int \Phi_1 \mu_1 dx_1 - { \sqrttwolagrsbat{1}  \int  \frac{\delta \cF[\qm_1]}{\delta \qm_1} \mu_1 dx_1 } -  \int \Phi_0 \mu_0 dx_0 + { \sqrttwolagrsbat{0} \int  \frac{\delta \cF[\qm_0]}{\delta \qm_0} \mu_0 dx_0} \nonumber  \\
% %   & -\int_0^1 \int  \Bigg( \frac{\partial \Phi_t }{\partial t}  +\frac{1}{2} \big\| \nabla \Phi_t \big\|^2  - \sqrttwolagrsbat{t}  \big\langle \nabla \Phi_t, \nabla  \frac{\delta \cF[\qm_t]}{\delta \qm_t} \big\rangle 
% % \Bigg) \qm_t dx_t dt \nonumber
% % \end{align}



% \textit{Lagrangian and Hamiltonian for Schrödinger Bridge:}
% %\subsubsection{Lagrangian and Hamiltonian for Schrödinger Bridge}
% % Consider the Wasserstein-2 kinetic energy $\cK[\qm_t, \dot{\qm}_t] = \frac{1}{2} \wmetricat{ \dot{\qm}_t, \dot{\qm}_t }{\qm_t}$ and potential energy 
% % \begin{align}
% % \begin{split}
% %     \cU[\qm_t, t] &=  -\lagrsbat{t} \wnormat{ 
% %     \gradw \cF[\qm_t]
% %     %\nabla \frac{\delta \cF}{\delta \qm_t}
% %     }{\qm_t} 
% %      +  \int \frac{\partial }{\partial t}\left(\sqrttwolagrsbat{t} \frac{\delta \cF[\qm_t]}{\delta \qm_t}\right) ~\qm_t~ dx_t, \quad  \\
% %      &= - \lagrsbat{t}  
% %        \int \|  \nabla \frac{\delta \cF[\qm_t]}{\delta \qm_t} \|^2 \qm_t dx_t +  \int \frac{\partial }{\partial t}\left(\sqrttwolagrsbat{t} \frac{\delta \cF[\qm_t]}{\delta \qm_t}\right) ~\qm_t~ dx_t,
% %     %\\
% %     % \cU[\qm_1, 1] &=  -\sqrttwolagrsbat{1} \int \frac{\delta \cF[\qm_1]}{\delta \qm_1} \mu_1 dx_1, \quad \text{and} \quad \cU[\qm_0, 0] =  \sqrttwolagrsbat{0}\int\frac{\delta \cF[\qm_0]}{\delta \qm_0} \mu_0 dx_0 ,
% %     \end{split}\label{eq:potential_sb}
% % \end{align}
% %  We note that the $\int \frac{\partial }{\partial t}\left(\sqrttwolagrsbat{t} \frac{\delta \cF[\qm_t]}{\delta \qm_t}\right)  \qm_t dx_t$ term in the potential energy is not necessary for the Schrödinger Bridge problem with time-independent diffusion coefficent, as presented in \cref{example:sb} (see \cref{example:sb_app} below).

As in \cref{prop:dual_obj}, the dual for the Wasserstein Lagrangian Flow with the Lagrangian in \cref{lemma:sb} involves the Hamiltonian in \cref{eq:gsb_hamiltonian}. %(see \cref{eq:expanded} below)
\begin{align}
%\cS_\cL(\{\mu_{0,1}\}) &=  \inf \limits_{\qm_t} \sup \limits_{\lagr_t} \int \lagr_1  \mu_1 dx_1 -  \int \lagr_0  \mu_0 dx_0 - \int_0^1  \left( \int \frac{\partial \lagr_t}{\partial t} \qm_t ~ dx_t+ \cH[\qm_t, \lagr_t, t] \right) dt  . \nonumber
\cS_\cL(&\{\mu_{0,1}\}) =  \inf \limits_{\qm_t} \sup \limits_{\lagr_t} \int \lagr_1  \mu_1 dx_1 -  \int \lagr_0  \mu_0 dx_0 \label{eq:expanded2} \\
&\phantom{\{\mu_{0,1}  \inf \limits_{\qm_t} \sup \limits_{\lagr_t}} - \int_0^1   \int \left( \frac{\partial \lagr_t}{\partial t} + \frac{1}{2}\int \| \nabla \lagr_t  \|^2 - \lagrsbat{t} \int \|  \nabla \frac{\delta \cF[\qm_t]}{\delta \qm_t} \|^2 + \frac{\partial }{\partial t}\left(\sqrttwolagrsbat{t} \frac{\delta \cF[\qm_t]}{\delta \qm_t}\right)  \right)  \qm_t ~ dx_t \nonumber
\end{align}
However, it is not clear how to optimize this objective in general due to the possibly non-linear term involving $ \nabla \frac{\delta \cF[\qm_t]}{\delta \qm_t}$ and $\frac{\partial }{\partial t}\left(\sqrttwolagrsbat{t} \frac{\delta \cF[\qm_t]}{\delta \qm_t}\right) $.
We will be able to derive a tractable (linear in $\qm_t$) dual objective for the classical \gls{SB} problem in \cref{example:sb_app} using a reparameterization in terms of the Fokker-Planck equation, or using the Hopf-Cole transform.  We derive the reparameterized dual in the following proposition, and show its relation with the generalized \gls{SB} problem.
%which will be helpful in linearizing the dual objective in \cref{eq:expanded2} for the classical \gls{SB} problem (\cref{example:sb_app}).   
%This is exactly the desired dual in the current proof (\cref{prop:sb}).


\begin{proposition}\label{prop:sb}
%Consider a Lagrangian defined using
The solution to the Wasserstein Lagrangian flow
\begin{align}
&\cS_{\cL}(\{\mu_{0,1}\}) = \inf
\limits_{\qm_t}
%\limits_{(\qm_t, \dot{\qm}_t)} 
\int_0^1 \mathcal{L}[\qm_t, \dot{\qm}_t,t]dt 
%\,\, \text{s.t. } \,\, &\dot{\qm}_t = - \langle \nabla, \qm_t \vel_t \rangle + \qm_t \action_t, \, 
%\\ \text{ and } \,\,  
\quad \st \quad
\qm_0 = \mu_0, \qquad \qm_1 = \mu_1 \label{eq:wlf_app} \\
% \end{align}
% using 
% \begin{align}
&\text{where}\,\,\,
 { \cK[\qm_t, \dot{\qm}_t, t] = \frac{1}{2} \wmetricat{ \dot{\qm}_t, \dot{\qm}_t }{\qm_t}, \,\,\, \cU[\qm_t, t] =  -\lagrsbat{t} \wnormat{ 
    \gradw \cF[\qm_t]
    }{\qm_t} 
     +  \int \frac{\partial }{\partial t}\left(\sqrttwolagrsbat{t} \frac{\delta \cF[\qm_t]}{\delta \qm_t}\right) \qm_t dx_t, } \nonumber % \\
     %&= - \lagrsbat{t}  
      % \int \|  \nabla \frac{\delta \cF[\qm_t]}{\delta \qm_t} \|^2 \qm_t dx_t +  \int \frac{\partial }{\partial t}\left(\sqrttwolagrsbat{t} \frac{\delta \cF[\qm_t]}{\delta \qm_t}\right) ~\qm_t~ dx_t, \nonumber
% \cL[\qm_t, \dot{\qm}_t, t] =  \frac{1}{2} \wmetricat{ \dot{\qm}_t, \dot{\qm}_t }{\qm_t} - \left( -\lagrsbat{t} \wnormat{ 
%     \gradw \cF[\qm_t]}{\qm_t} +  \int \frac{\partial }{\partial t}\left(\sqrttwolagrsbat{t} \frac{\delta \cF[\qm_t]}{\delta \qm_t}\right) ~\qm_t~ dx_t \right).
\end{align}

matches the solution to the generalized \gls{SB} problem in \cref{eq:gsb} up to a constant $c(\mu_{0,1})$ wrt $\qm_t$,
\begin{align}
\cS_{gSB}(\{\mu_{0,1}\}) = \cS_\cL(\{\mu_{0,1}\}) + c(\{\mu_{0,1}\}). 
\end{align}
Further, $\cS  = \cS_{gSB}(\{\mu_{0,1}\}) = \cS_\cL(\{\mu_{0,1}\}) + c(\{\mu_{0,1}\}) $ is the solution to the (dual) optimization
\small
\begin{align}
\cS &=  \inf \limits_{\qm_t} \sup \limits_{\Phi_t}  \int \Phi_1 \mu_1 dx_1  -  \int \Phi_0 \mu_0 dx_0  %\nonumber  \\
  %& 
  -\int_0^1 \int  \Bigg( \frac{\partial \Phi_t }{\partial t}  +\frac{1}{2} \big\| \nabla \Phi_t \big\|^2  - \sqrttwolagrsbat{t}  \big\langle \nabla \Phi_t, \nabla  \frac{\delta \cF[\qm_t]}{\delta \qm_t} \big\rangle 
\Bigg) \qm_t dx_t dt . \label{eq:gsb_final}
\end{align}
\normalsize
Thus, we have obtained a dual objective for the WLF in \cref{eq:wlf_app} which is linear in $\qm_t$.
\end{proposition}
\begin{proof}
%\textit{Fokker-Planck Reparameterization:} %Hopf-Cole Transform}
We first consider a Fokker-Planck reparameterization
\begin{align}
     \lagr_t = \Phi_t - \sqrttwolagrsbat{t}  \frac{\delta \cF[\qm_t]}{\delta \qm_t}, \qquad \qquad \nabla \lagr_t  =  \nabla \Phi_t- \sqrttwolagrsbat{t} \nabla \frac{\delta \cF[\qm_t]}{\delta \qm_t} . \label{eq:reparam_sb}
\end{align}
Noting that $\lagr_t$ corresponds to the continuity equation in \cref{eq:hamil_sb}, $\dot{\qm}_t = -\langle \nabla, \qm_t \nabla \lagr_t \rangle$.   Via the above reparameterization, we see that $\nabla \Phi_t $ corresponds to the drift in the Fokker-Planck dynamics for the generalized \gls{SB} problem in \cref{eq:gsb}, 
%$\dot{\qm}_t =  -\langle \nabla, \qm_t \nabla \Phi_t \rangle - \sqrttwolagrsbat{t} \langle \nabla, \qm_t \nabla \log \qm_t \rangle = -\langle \nabla, \qm_t \nabla \Phi_t \rangle + \sqrttwolagrsbat{t} \Delta \qm_t$.   
% For general gradient-flow dynamics as in \cref{eq:gsb}, we have 
$ \dot{\qm}_t=  -\langle \nabla, \qm_t \nabla \Phi_t \rangle + \sqrttwolagrsbat{t} \langle \nabla, \qm_t \nabla \frac{\delta  \cF[\qm_t]}{\delta \qm_t} \rangle~$.

%which will allow us to linearize the objective in \cref{eq:gsb_hamiltonian} for the case of the classical \textsc{sb} problem.



% To understand this reparameterization, note that for classical \textsc{sb} problem with $\cF[\qm_t] = -H[\qm_t]$, we have $\nabla \frac{\delta \cF[\qm_t]}{\delta \qm_t} = \nabla \log \qm_t$ (see \cref{example:sb_app} below).   Recalling that the dynamics corresponding to $\lagr_t$ follow the continuity equation, $\nabla \lagr_t =  \nabla \Phi_t - \sqrttwolagrsbat{t} \nabla \log  \qm_t $ corresponds to the drift of the \textit{probability flow \textsc{ode}} \citep{song2020score}.   Substituting into the continuity equation $\dot{\qm}_t = -\langle \nabla, \qm_t \nabla \lagr_t \rangle$ and simplifying, we see that $\nabla \Phi_t $ corresponds to the drift in the Fokker Planck equation $\dot{\qm}_t =  -\langle \nabla, \qm_t \nabla \Phi_t \rangle - \sqrttwolagrsbat{t} \langle \nabla, \qm_t \nabla \log \qm_t \rangle = -\langle \nabla, \qm_t \nabla \Phi_t \rangle + \sqrttwolagrsbat{t} \Delta \qm_t$.   
% For general gradient-flow dynamics as in \cref{eq:gsb}, we have $ \dot{\qm}_t=  -\langle \nabla, \qm_t \nabla \Phi_t \rangle + \sqrttwolagrsbat{t} \langle \nabla, \qm_t \nabla \frac{\delta  \cF[\qm_t]}{\delta \qm_t} \rangle~$\citep{leger2021hopf}.

\textit{Wasserstein Lagrangian Dual Objective in the Fokker-Planck Reparameterization:}
Starting from the dual objective in \cref{eq:expanded2}, we perform the reparameterization in \cref{eq:reparam_sb}, $\lagr_t = \Phi_t - \sqrttwolagrsbat{t}  \frac{\delta \cF[\qm_t]}{\delta \qm_t}$,
\begin{align}
\cS_\cL(\{\mu_{0,1}\}) &= \inf \limits_{\qm_t} \sup \limits_{\Phi_t}  \int \Phi_1 \mu_1 dx_1 - { \sqrttwolagrsbat{1}  \int  \frac{\delta \cF[\qm_1]}{\delta \qm_1} \mu_1 dx_1 } -  \int \Phi_0 \mu_0 dx_0 + { \sqrttwolagrsbat{0} \int  \frac{\delta \cF[\qm_0]}{\delta \qm_0} \mu_0 dx_0} \nonumber \\
&\phantom{\inf \limits_{\qm_t} \sup \limits_{\lagr_t}} -\int_0^1 \int  \Bigg( \frac{\partial \Phi_t }{\partial t}  - \cancel{\frac{\partial }{\partial t}\left(\sqrttwolagrsbat{t}    \frac{\delta \cF[\qm_t]}{\delta \qm_t} \right) } + \cancel{\frac{\partial }{\partial t}\left(  \sqrttwolagrsbat{t}  \frac{\delta \cF[\qm_t]}{\delta \qm_t} \right) } \nonumber \\
& \phantom{ \inf \limits_{\qm_t} \sup \limits_{\lagr_t}} +\frac{1}{2} \left\langle \nabla \Phi_t - \sqrttwolagrsbat{t} \nabla  \frac{\delta \cF[\qm_t]}{\delta \qm_t}, \nabla \Phi_t - \sqrttwolagrsbat{t} \nabla  \frac{\delta \cF[\qm_t]}{\delta \qm_t} \right\rangle -
\lagrsbat{t} \left\| \nabla \frac{\delta \cF[\qm_t]}{\delta \qm_t}\right\|^2
\Bigg) \qm_t ~ dx_t dt \nonumber %\label{eq:gsb_final}
\end{align}
yielding the reparameterized dual objective as
\begin{align}
\cS_\cL(\{\mu_{0,1}\}) &=  \inf \limits_{\qm_t} \sup \limits_{\Phi_t}  \int \Phi_1 \mu_1 dx_1 - { \sqrttwolagrsbat{1}  \int  \frac{\delta \cF[\qm_1]}{\delta \qm_1} \mu_1 dx_1 } -  \int \Phi_0 \mu_0 dx_0 + { \sqrttwolagrsbat{0} \int  \frac{\delta \cF[\qm_0]}{\delta \qm_0} \mu_0 dx_0} \nonumber  \\
  & -\int_0^1 \int  \Bigg( \frac{\partial \Phi_t }{\partial t}  +\frac{1}{2} \big\| \nabla \Phi_t \big\|^2  - \sqrttwolagrsbat{t}  \big\langle \nabla \Phi_t, \nabla  \frac{\delta \cF[\qm_t]}{\delta \qm_t} \big\rangle 
\Bigg) \qm_t dx_t dt \nonumber
\end{align}
where the Hamiltonian now matches Eq. 7 in \citet{leger2021hopf}.
 
Finally, we consider adding terms  $c(\mu_{0,1}) = \sqrttwolagrsbat{1}  \int  \frac{\delta \cF[\mu_1]}{\delta \mu_1} \mu_1 dx_1 -\sqrttwolagrsbat{0}  \int  \frac{\delta \cF[\mu_0]}{\delta \mu_0} \mu_0 dx_0 $ which are constant with respect to $\qm_{0,1}$,
\begin{align}
\cS_\cL(\{\mu_{0,1}\}) + c(\mu_{0,1}) &=  \inf \limits_{\qm_t} \sup \limits_{\Phi_t}  \int \Phi_1 \mu_1 dx_1 + { \sqrttwolagrsbat{1}  \int \left( \frac{\delta \cF[\mu_1]}{\delta \mu_1} - \frac{\delta \cF[\qm_1]}{\delta \qm_1} \right) \mu_1 dx_1 } \label{eq:wlf_dual_sb} \\
&\phantom{ \inf \limits_{\qm_t} \sup \limits_{\Phi_t} } -  \int \Phi_0 \mu_0 dx_0 -  \sqrttwolagrsbat{0} \int  \left( \frac{\delta \cF[\mu_0]}{\delta \mu_0} - \frac{\delta \cF[\qm_0]}{\delta \qm_0} \right)\mu_0  dx_0  \nonumber \\
  &\phantom{ \inf \limits_{\qm_t} \sup \limits_{\Phi_t} } -\int_0^1 \int  \Bigg( \frac{\partial \Phi_t }{\partial t}  +\frac{1}{2} \big\| \nabla \Phi_t \big\|^2  - \sqrttwolagrsbat{t}  \big\langle \nabla \Phi_t, \nabla  \frac{\delta \cF[\qm_t]}{\delta \qm_t} \big\rangle 
\Bigg) \qm_t dx_t dt \nonumber
\end{align}
We will argue that the endpoint terms can be ignored without affecting the optimal value of the optimization.   
Intuitively, $\frac{\delta \cF[\mu_1]}{\delta \mu_1} - \frac{\delta \cF[\qm_1]}{\delta \qm_1}$ and $\frac{\delta \cF[\mu_0]}{\delta \mu_0} - \frac{\delta \cF[\qm_0]}{\delta \qm_0}$ will cancel if $\qm_1= \mu_1 $ and $\qm_0 = \mu_0$, which is guaranteed at the optimum of \cref{eq:wlf_app}. 
We first derive the dual of the generalized \gls{SB} problem before showing the equivalence $\cS_{gSB}(\{\mu_{0,1}\})  = \cS_\cL(\{\mu_{0,1}\}) + c(\mu_{0,1})$.

%We now show that the dual in \cref{eq:wlf_dual_sb} corresponds to the solution to the generalized \gls{SB} problem.

% \begin{align}
% \cS_{\cL}(\{\mu_{0,1}\}) = \inf
% \limits_{\qm_t}
% %\limits_{(\qm_t, \dot{\qm}_t)} 
% \int_0^1 \mathcal{L}[\qm_t, \dot{\qm}_t,t]dt 
% %\,\, \text{s.t. } \,\, &\dot{\qm}_t = - \langle \nabla, \qm_t \vel_t \rangle + \qm_t \action_t, \, 
% %\\ \text{ and } \,\,  
% \quad \st \quad
% \qm_0 = \mu_0, \qquad \qm_1 = \mu_1
% \end{align}


\textit{Generalized Schrödinger Bridge Dual Objective:}
Consider the optimization in \cref{eq:gsb}
\small 
\begin{align}
\cS_{gSB}(\{\mu_{0,1}\}) = \inf \limits_{\qm_t, v_t}
\int_0^1 
 \frac{1}{2} \| v_t \|^2 \qm_t dx_t
 \st \dot{\qm}_t  &= -\langle \nabla, \qm_t \vel_t \rangle + \sqrttwolagrsbat{t} \langle \nabla, \qm_t ~\nabla \frac{\delta \cF}{\delta \qm_t} \rangle,\,  \qm_0 = \mu_0, \,\, \qm_1 = \mu_1  
\nonumber
\end{align}
\normalsize
Introducing Lagrange multipliers $\lambda_0, \lambda_1$ to enforce the endpoint constraints and $\Phi_t$ to enforce the dynamics constraint, 
%we follow similar derivations as in the proof of \cref{prop:dual_obj}-\ref{prop:dual_obj_app} a
\small 
\begin{align}
\cS_{gSB}(\{\mu_{0,1}\}) &= \inf \limits_{\qm_t, v_t} \sup\limits_{\Phi_t, \lambda_{0,1}}
\int_0^1 \frac{1}{2} \| v_t \|^2 \qm_t dx_t
 + \int \Phi_t \left( \dot{\qm}_t + \langle \nabla, \qm_t \vel_t \rangle - \sqrttwolagrsbat{t} \langle \nabla, \qm_t ~\nabla \frac{\delta \cF}{\delta \qm_t} \rangle\right) dx_t \label{eq:gsb11} \\
 &\phantom{=\inf \limits_{\qm_t, v_t} \sup\limits_{\Phi_t, \lambda_{0,1}}} + \int \lambda_1 \left(\qm_1 - \mu_1  \right) dx_1 + \int \lambda_0 \left(\qm_0 - \mu_0 \right) dx_0 \nonumber \\
&= \inf \limits_{\qm_t, v_t} \sup\limits_{\Phi_t, \lambda_{0,1}}
\int_0^1 \frac{1}{2} \| v_t \|^2 \qm_t dx_t + \int \Phi_1 \qm_1 dx_1 - \int \Phi_0 \qm_0 dx_0
 - \int_0^1 \int \frac{\partial \Phi_t}{\partial t} \qm_t dx_t dt \\
 &\phantom{=} - \int_0^1 \int  \left\langle \nabla \Phi_t, \vel_t - \sqrttwolagrsbat{t} \nabla \frac{\delta \cF}{\delta \qm_t} \right \rangle \qm_t dx_t dt 
 %\\&\phantom{=\inf \limits_{\qm_t, v_t} \sup\limits_{\Phi_t, \lambda_{0,1}}} 
 + \int \lambda_1 \left(\qm_1 - \mu_1  \right) dx_1 + \int \lambda_0 \left(\qm_0 - \mu_0 \right) dx_0 \nonumber
\end{align}
\normalsize
Eliminating $\lambda_{0,1}$ implies $\lambda_1 = \Phi_1$ and $\lambda_0 = \Phi_0$, whereas eliminating $v_t$ implies $v_t = \nabla \Phi_t$,
\small 
\begin{align}
\cS_{gSB}(\{\mu_{0,1}\}) &= 
\inf \limits_{\qm_t} \sup\limits_{\Phi_t}
\int \Phi_1 \mu_1 dx_1 - \int \Phi_0 \mu_0 dx_0 - \int_0^1 \left( \frac{\partial \Phi_t}{\partial t} + \frac{1}{2} \| \Phi_t \|^2 
- \sqrttwolagrsbat{t} \left\langle \nabla \Phi_t, \nabla \frac{\delta \cF}{\delta \qm_t} \right\rangle
\right) \qm_t dx_t \label{eq:dual_gsb}
\end{align}
\normalsize

\textit{Wasserstein Lagrangian vs. Generalized Schrödinger Bridge:}
Finally, to show that $\cS_{gSB}(\{\mu_{0,1}\})  = \cS_\cL(\{\mu_{0,1}\}) + c(\mu_{0,1})$, we note that 
\begin{align}
%\begin{aligned}
\cS_{gSB}(\{\mu_{0,1}\}) -c(\mu_{0,1})  &= \inf \limits_{\qm_t, v_t}
\int_0^1 
 \frac{1}{2} \| v_t \|^2 \qm_t dx_t  - \sqrttwolagrsbat{1}  \int \left( \frac{\delta \cF[\mu_1]}{\delta \mu_1} - \frac{\delta \cF[\qm_1]}{\delta \qm_1} \right) \mu_1 dx_1 \label{eq:gsb_minus} \\
 &\phantom{= \inf \limits_{\qm_t, v_t} \int_0^1 
 \frac{1}{2} \| v_t \|^2 \qm_t dx_t} +  \sqrttwolagrsbat{0} \int  \left( \frac{\delta \cF[\mu_0]}{\delta \mu_0} - \frac{\delta \cF[\qm_0]}{\delta \qm_0} \right)\mu_0  dx_0 \nonumber \\
 &\quad \st \,\, \dot{\qm}_t  = -\langle \nabla, \qm_t \vel_t \rangle + \sqrttwolagrsbat{t} \langle \nabla, \qm_t ~\nabla \frac{\delta \cF}{\delta \qm_t} \rangle, \,\,\,  \qm_0 = \mu_0, \,\, \qm_1 = \mu_1 \nonumber \\
 &= \cS_{gSB}(\{\mu_{0,1}\}) \label{eq:gsb_const_equal}
\end{align}
matches the value of $\cS_{gSB}(\{\mu_{0,1}\}) $ since $\qm_0 = \mu_0$ and $\qm_1 = \mu_1$ at optimality.   We note that the endpoint terms are unaffected by the same derivations as above to derive the dual \cref{eq:dual_gsb} from \cref{eq:gsb11}, which yields the dual of \cref{eq:gsb_minus} as
\small
\begin{align}
\cS_{gSB}(\{\mu_{0,1}\}) -c(\mu_{0,1}) &=  \inf \limits_{\qm_t} \sup \limits_{\Phi_t}  \int \Phi_1 \mu_1 dx_1 + { \sqrttwolagrsbat{1}  \int \left( \frac{\delta \cF[\mu_1]}{\delta \mu_1} - \frac{\delta \cF[\qm_1]}{\delta \qm_1} \right) \mu_1 dx_1 } \label{eq:wlf_dual_sb} \\
&\phantom{ \inf \limits_{\qm_t} \sup \limits_{\Phi_t} } -  \int \Phi_0 \mu_0 dx_0 -  \sqrttwolagrsbat{0} \int  \left( \frac{\delta \cF[\mu_0]}{\delta \mu_0} - \frac{\delta \cF[\qm_0]}{\delta \qm_0} \right)\mu_0  dx_0  \nonumber \\
  &\phantom{ \inf \limits_{\qm_t} \sup \limits_{\Phi_t} } -\int_0^1 \int  \Bigg( \frac{\partial \Phi_t }{\partial t}  +\frac{1}{2} \big\| \nabla \Phi_t \big\|^2  - \sqrttwolagrsbat{t}  \big\langle \nabla \Phi_t, \nabla  \frac{\delta \cF[\qm_t]}{\delta \qm_t} \big\rangle 
\Bigg) \qm_t dx_t dt \nonumber \\
&= \cS_\cL(\{\mu_{0,1}\}) + c(\mu_{0,1}) \label{eq:wlf_const_equal}
\end{align}
\normalsize
where we recognize the dual as matching the one obtained for $\cS_\cL(\{\mu_{0,1}\}) + c(\mu_{0,1})$ in \cref{eq:wlf_dual_sb}.  Thus, \cref{eq:gsb_const_equal} and \cref{eq:wlf_const_equal} imply $\cS_\cL(\{\mu_{0,1}\}) + c(\mu_{0,1}) = \cS_{gSB}(\{\mu_{0,1}\})$ as desired (since both are equal to $\cS_{gSB}(\{\mu_{0,1}\}) -c(\mu_{0,1})$).
\end{proof}

\subsubsection{Generalized Schrödinger Bridge Examples}
%\Kirill{i think it's not only Schrodinger Bridge}

\begin{example}[\textbf{Schrödinger Bridge with Time-Dependent Diffusion Coefficient}]\label{example:sb_app}
Choosing $\cF[\qm_t] = -H[\qm_t]$, we have $\nabla \frac{\delta \cF[\qm_t]}{\delta \qm_t} = \nabla \log \qm_t$. 
Simplifying and integrating by parts, the final term in \cref{eq:gsb_final} or \cref{eq:dual_gsb} becomes
\begin{align}
\int_0^1 \int  \big\langle \nabla \Phi_t, \nabla \log \qm_t \big\rangle 
 \qm_t dx_t dt = \int_0^1 \int  \big\langle \nabla \Phi_t, \nabla \qm_t \big\rangle 
 dx_t dt = - \int_0^1 \int \left( \Delta \Phi_t \right) ~ \qm_t~ dx_t dt 
\end{align}
which yields the eventual dual objective
\begin{align}
 \hspace*{-.2cm} \cS_{SB} = \sup \limits_{\Phi_t} \inf \limits_{\qm_t} ~ \int \Phi_1 d\mu_1 
  -  \int \Phi_0 d\mu_0   -\int_0^1 \int  \Bigg( \frac{\partial \Phi_t }{\partial t}  +\frac{1}{2} \big\| \nabla \Phi_t \big\|^2  + \sqrttwolagrsbat{t}  \Delta \Phi_t
\Bigg) \qm_t dx_t dt \label{appeq:sb_t_final}.
\end{align}
\end{example}

%\subsubsection{Schrödinger Bridge Examples}
\begin{example}[\textbf{Schrödinger Bridge with Time-Independent Diffusion Coefficient}]
When $\sqrttwolagrsbat{}$ is independent of $t$, the additional term $\int \frac{\partial }{\partial t}\left( \sqrttwolagrsbat{} \frac{\delta \cF[\qm_t]}{\delta \qm_t}\right)~\qm_t~ dx_t$ in the potential energy in \cref{prop:sb} vanishes for the entropy functional, with $\frac{\delta \cF[\qm_t]}{\delta \qm_t} = \log \qm_t$ and
\begin{align}
\int \frac{\partial }{\partial t}\left( \sqrttwolagrsbat{} \frac{\delta \cF[\qm_t]}{\delta \qm_t}\right)~\qm_t~ dx_t = \sqrttwolagrsbat{} \int   \frac{\partial \log \qm_t}{\partial t}~\qm_t~ dx_t = \sqrttwolagrsbat{} \frac{\partial }{\partial t} \int    \qm_t~ dx_t = 0 .
\end{align}
Note that this observation simplifies the potential energy and derivations above, but preserves the same dual objective from \cref{appeq:sb_t_final}.
\end{example}

\begin{example}[Porous Medium Dynamics \citep{otto2001geometry, leger2021hopf}]\label{example:porous}
Consider the (scaled) negative Tsallis entropy $\cF[\qm_t] = -H_\alpha[\qm_t] =  \frac{1}{(q-1)} \int \qm_t^{q} dx_t$ .   In this case, we have
\begin{align}
\frac{\delta \cF[\qm_t]}{\delta \qm_t} = \frac{q}{q-1} \qm_t(x_t)^{q-1} \qquad \qquad \nabla \frac{\delta \cF[\qm_t]}{\delta \qm_t} =  q ~ \qm_t(x_t)^{q-2}  \nabla \qm_t(x_t)
\end{align}
Reparameterizing the continuity equation with \cref{eq:reparam_sb} yields a non-linear Fokker-Planck equation with $q$-Brownian motion, after simplifying $q \langle \nabla, \qm_t \qm_t^{q-2}  \nabla \qm_t \rangle = q \langle \nabla,  \qm_t^{q-1}  \nabla  \qm_t \rangle = \langle \nabla, \nabla \qm_t^{q}\rangle = \Delta \qm_t^q$,
\begin{align}
 \text{For} \,\, \nabla \lagr_t  =  \nabla \Phi_t- \sqrttwolagrsbat{t} q ~ \qm_t^{q-2} \nabla \qm_t , \quad \text{and} \quad\dot{\qm}_t &= -\langle \nabla, \qm_t \nabla \phi_t \rangle \qquad  \nonumber \\
 \implies \quad \dot{\qm}_t &= -\langle \nabla, \qm_t \nabla \Phi_t \rangle + \sqrttwolagrsbat{t} q \langle \nabla, \qm_t \qm_t^{q-2}  \nabla \qm_t \rangle  \nonumber \\
 \implies \quad \dot{\qm}_t &= -\langle \nabla, \qm_t \nabla \Phi_t \rangle + \sqrttwolagrsbat{t} \Delta \qm_t^q.
\end{align}
For the appropriate potential energy in \cref{prop:sb}, we apply similar simplifications to the final term in \cref{eq:gsb_final} or \cref{eq:dual_gsb}
\begin{align}
  \int_0^1 \int \sqrttwolagrsbat{t}  q \big\langle \nabla \Phi_t, \qm_t^{q-2}  \nabla \qm_t  \big\rangle 
 \qm_t dx_t dt 
 &= \int_0^1 \int \sqrttwolagrsbat{t}  \big\langle \nabla \Phi_t, \frac{q}{q} \nabla \qm_t^q \big\rangle  dx_t dt
 = - \int_0^1 \int \sqrttwolagrsbat{t}   ( \Delta \Phi_t ) \qm_t^q  dx_t dt \nonumber
\end{align}
Substituting back into \cref{eq:gsb_final} or \cref{eq:dual_gsb}, 
\begin{align}
 \cS_{PM} = \sup \limits_{\Phi_t} \inf \limits_{\qm_t} ~ \int \Phi_1 d\mu_1 
  -  \int \Phi_0 d\mu_0   -\int_0^1 \int  \Bigg( \frac{\partial \Phi_t }{\partial t}  +\frac{1}{2} \big\| \nabla \Phi_t \big\|^2  + \sqrttwolagrsbat{t} ( \Delta \Phi_t ) \qm_t^{q-1}  
\Bigg) \qm_t dx_t dt \nonumber
%\label{eq:gsb_final}
\end{align}
In contrast to the case of $q=1$, we have a nonlinear term in the density $\qm_t^{q-1}$, which cannot be optimized simply by drawing samples from $\qm_t$ and thus is not immediately tractable under our proposed framework.
\end{example}


==> text/background.tex <==
\subsection{Wasserstein Lagrangian Mechanics}

We consider the following optimization problem

\begin{align}
    \underbrace{S(p_0, p_1)}_{\text{total action}} = \inf_{q_t,s_t} \int dtdx\; \underbrace{\mathcal{L}(q_t,s_t,t)}_{\text{Lagrangian}},
    \;\;\text{ s.t. }\;\; \dot{q}_t = -\inner{\nabla}{q_t v_t}, q_0 = p_0, q_1 = p_1.
\end{align}

\begin{align}
    \underbrace{S(p_0, p_1)}_{\text{total action}} = \inf_{q_t,v_t} \underbrace{\int dtdx\; q_t \frac{1}{2}\norm{v_t}^2}_{\text{kinetic energy}} - \underbrace{\int dtdx\; U(q_t)}_{\text{potential energy}},
    \;\;\text{ s.t. }\;\; \dot{q}_t = -\inner{\nabla}{q_t v_t}, q_0 = p_0, q_1 = p_1.
\end{align}
\Kirill{introduce the growth term and the parameter balancing between transportation and teleportation.}

The only difference with classical Lagrangian mechanics is that potential energy now can depend on the current density $q_t$. 
In other words, potential energy now is defined on the Wasserstein Manifold $\mathcal{U}: \mathcal{P}_2(X) \to \mathbb{R}$. 
Choosing different potential functionals, this formulation yields following problems.

\paragraph{Optimal Transport (OT)}
\begin{align}\label{eq:bb_ot}
    \inf_{q_t,v_t} \int dtdx\; q_t \frac{1}{2}\norm{v_t}^2,
    \;\;\text{ s.t. }\;\; \dot{q}_t = -\inner{\nabla}{q_t v_t}, \;\; q_0 = p_0, \;\; q_1 = p_1.
\end{align}

\paragraph{Physically constrained OT}
\begin{align}
    \inf_{q_t,v_t} \int dtdx\; q_t \left[\frac{1}{2}\norm{v_t}^2 - V_t \right],
    \;\;\text{ s.t. }\;\; \dot{q}_t = -\inner{\nabla}{q_t v_t}, \;\; q_0 = p_0, \;\; q_1 = p_1.
\end{align}

\paragraph{Unbalanced OT}
\begin{align}\label{eq:uot}
    \inf_{q_t,v_t,g_t} \int dtdx\; q_t \left[\frac{1}{2}\norm{v_t}^2+\frac{1}{2}g_t^2\right],
    \;\;\text{ s.t. }\;\; \dot{q}_t = -\inner{\nabla}{q_t v_t} + g_tq_t, \;\; q_0 = p_0, \;\; q_1 = p_1.
\end{align}

\paragraph{Entropy regularized OT (Schrödinger Bridge)}
\begin{align}\label{eq:sb}
    \inf_{q_t,v_t} \int dtdx\; q_t \left[\frac{1}{2}\norm{v_t}^2 + \frac{\sigma_t^4}{8}\norm{\nabla\log q_t}^2\right],
    \;\;\text{ s.t. }\;\; \dot{q}_t = -\inner{\nabla}{q_t v_t}, \;\; q_0 = p_0, \;\; q_1 = p_1.
\end{align}

\paragraph{Optimal control}
\begin{align}\label{eq:sb}
    \inf_{q_t,A_t} \int dtdxdv\; q_t(x,v) \left[\frac{1}{2}\norm{A_t(x,v)}^2\right],
    \;\;\text{ s.t. }\;\; \dot{q}_t(x,v) = -\inner{\nabla_x}{q_t(x,v) v} - \inner{\nabla_v}{q_t(x,v) A(x,v)}, \\
    q_0 = p_0, \;\; q_1 = p_1.
\end{align}

\begin{table}[t]
    \caption{Examples}
    \label{tab:examples}
    \begin{center}
    \begin{tabular}{llll}
         \multicolumn{1}{c}{\bf Problem} & \multicolumn{1}{c}{\bf Lagrangian} & \multicolumn{1}{c}{\bf Dual} & \multicolumn{1}{c}{\bf cont}
         \\ \hline \\
         OT & $q_t \frac{1}{2}\norm{v_t}^2$ & $\int s_0p_0 - \int s_1 p_1 - \int q_t\left[\frac{1}{2}\norm{\nabla s_t}^2 + \deriv{s_t}{t}\right]$ & $\dot{q}_t = -\inner{\nabla}{q_t v_t}$  \\
         physical OT & $q_t \left[\frac{1}{2}\norm{v_t}^2 - V_t \right]$ & $\int s_0p_0 - \int s_1 p_1 - \int q_t\left[\frac{1}{2}\norm{\nabla s_t}^2 + \deriv{s_t}{t} + V_t\right]$ & $\dot{q}_t = -\inner{\nabla}{q_t v_t}$ \\
         Unbalanced OT & $q_t \left[\frac{1}{2}\norm{v_t}^2+\frac{1}{2}g_t^2\right]$ && $\dot{q}_t = -\inner{\nabla}{q_t v_t} + g_t q_t$ \\
         Schrodinger Bridge & $q_t \left[\frac{1}{2}\norm{v_t}^2 + \frac{\sigma_t^4}{8}\norm{\nabla\log q_t}^2\right]$ && $\dot{q}_t = -\inner{\nabla}{q_t v_t}$\\
    \end{tabular}
    \end{center}
\end{table}

==> text/old_proofs.tex <==
\section{Computational methods' proofs}

\subsection{Optimal Transport}\label{app:ot}
\begin{proposition*}
Optimization problem from \cref{eq:bb_ot} is equivalent to
\begin{align}
\begin{split}
    \mathcal{L} = \sup_{s_t(x)}  \inf_{q_t(x)} \; \int dx\; s_1(x) p_1(x) -\int dx\; s_0(x) p_0(x) -  \int \limits_0^1 \int \limits_{\mathcal{X}} dt dx \; q_t(x) \;\bigg[\frac{1}{2} \| \nabla s_t(x) \|^2 + \deriv{s_t(x)}{t}\bigg]\,,
\end{split}
\end{align}
and at the optimum we have
\begin{align}
    \deriv{q_t(x)}{t} = - \inner{\nabla}{q_t(x)\nabla s_t(x)}, \;\; q_0 = p_0, \;\; q_1 = p_1, \;\; \text{ and }\;\; \frac{1}{2} \| \nabla s_t(x) \|^2 + \deriv{s_t(x)}{t} = 0.
\end{align}
\end{proposition*}
\begin{proof}
We start with the Lagrangian
\begin{align}
\begin{split}
    \mathcal{L} = \sup_{\lambda_t(x)} \inf_{q_t(x), v_t(x)} & \; \int \limits_0^1 \int \limits_{\mathcal{X}} dt dx \; q_t(x) \frac{1}{2} \norm{v_t(x)}^2 + \int \limits_0^1 \int \limits_{\mathcal{X}} dt dx \; \lambda_t(x) \bigg[  \frac{\partial q_t(x) }{\partial t}  + \inner{\nabla}{q_t(x) v_t(x)} \bigg] \\
    & + \int dx\; \lambda_1(x) \bigg( p_1(x) - q_1(x) \bigg) -\int dx\; \lambda_0(x) \bigg( p_0(x) - q_0(x) \bigg).
\end{split}
\end{align}
The first order condition for $v_t$ then yields $v_t = \nabla \lambda_t$.
Renaming $\lambda_t$ as $s_t$, we have
\begin{align}
\begin{split}
    \mathcal{L} = \sup_{s_t(x)}  \inf_{q_t(x)} & \;  \int \limits_0^1 \int \limits_{\mathcal{X}} dt dx \; q_t(x) \; \frac{1}{2} \| \nabla s_t(x) \|^2  + \int \limits_0^1 \int \limits_{\mathcal{X}} dt dx \; s_t(x) \left[  \frac{\partial q_t(x) }{\partial t}  + \langle \nabla, q_t(x) \nabla s_t(x) \rangle \right] \\
    & + \int dx\; s_1(x) \bigg( p_1(x) - q_1(x) \bigg) -\int dx\; s_0(x) \bigg( p_0(x) - q_0(x) \bigg).
\end{split}
\end{align}
Taking the second term by parts we get
\begin{align}
\begin{split}
    \mathcal{L} = \sup_{s_t(x)}  \inf_{q_t(x)} \; \int dx\; s_1(x) p_1(x) -\int dx\; s_0(x) p_0(x) -  \int \limits_0^1 \int \limits_{\mathcal{X}} dt dx \; q_t(x) \;\bigg[\frac{1}{2} \| \nabla s_t(x) \|^2 + \deriv{s_t(x)}{t}\bigg].
\end{split}
\end{align}
The first order condition for $q_t$ is
\begin{align}
    \nabla\bigg[\frac{1}{2} \| \nabla s_t(x) \|^2 + \deriv{s_t(x)}{t}\bigg] = 0.
\end{align}
The first order condition for $s_t$ yields
\begin{align}
    \deriv{q_t(x)}{t} = - \inner{\nabla}{q_t(x)\nabla s_t(x)}, \;\; q_0 = p_0, \;\; q_1 = p_1.
\end{align}
\end{proof}

\subsection{Unbalanced OT}\label{app:uot}
\begin{proposition*}
Optimization problem from \cref{eq:uot} is equivalent to
\begin{align}
\begin{split}
    \mathcal{L} = \sup_{s_t(x)}  \inf_{q_t(x)} \; \int dx\; s_1(x) p_1(x) -\int dx\; s_0(x) p_0(x) -  \int \limits_0^1 \int \limits_{\mathcal{X}} dt dx \; q_t(x) \;\bigg[\frac{1}{2} \| \nabla s_t(x) \|^2 + \frac{1}{2}s_t(x)^2 + \deriv{s_t(x)}{t}\bigg]\,,
\end{split}
\end{align}
and at the optimum we have
\begin{align}
    \deriv{q_t(x)}{t} = - \inner{\nabla}{q_t(x)\nabla s_t(x)} + s_t(x)q_t(x), \;\; q_0 = p_0, \;\; q_1 = p_1, \;\; \text{ and }\;\; \frac{1}{2} \| \nabla s_t(x) \|^2 + \frac{1}{2}s_t(x)^2 + \deriv{s_t(x)}{t} = 0.
\end{align}
\end{proposition*}
\begin{proof}
We start with the Lagrangian
\begin{align}
\begin{split}
    \mathcal{L} = \sup_{\lambda_t(x)} \inf_{q_t(x), v_t(x)} & \; \int \limits_0^1 \int \limits_{\mathcal{X}} dt dx \; q_t(x) \left[\frac{1}{2} \norm{v_t(x)}^2 + \frac{1}{2}g_t(x)^2\right] + \int \limits_0^1 \int \limits_{\mathcal{X}} dt dx \; \lambda_t(x) \bigg[  \frac{\partial q_t(x) }{\partial t}  + \inner{\nabla}{q_t(x) v_t(x)} - q_t(x)g_t(x)\bigg] \\
    & + \int dx\; \lambda_1(x) \bigg( p_1(x) - q_1(x) \bigg) -\int dx\; \lambda_0(x) \bigg( p_0(x) - q_0(x) \bigg).
\end{split}
\end{align}
The first order condition for $v_t, g_t$ then yields $v_t = \nabla \lambda_t$ and $g_t = \lambda_t$.
Renaming $\lambda_t$ as $s_t$, we have
\begin{align}
\begin{split}
    \mathcal{L} = \sup_{s_t(x)}  \inf_{q_t(x)} & \;  \int \limits_0^1 \int \limits_{\mathcal{X}} dt dx \; q_t(x) \; \left[\frac{1}{2} \norm{\nabla s_t(x)}^2 + \frac{1}{2}s_t(x)^2\right]  + \int \limits_0^1 \int \limits_{\mathcal{X}} dt dx \; s_t(x) \left[  \frac{\partial q_t(x) }{\partial t}  + \langle \nabla, q_t(x) \nabla s_t(x) \rangle - s_t(x)q_t(x) \right] \\
    & + \int dx\; s_1(x) \bigg( p_1(x) - q_1(x) \bigg) -\int dx\; s_0(x) \bigg( p_0(x) - q_0(x) \bigg).
\end{split}
\end{align}
Taking the second term by parts we get
\begin{align}
\begin{split}
    \mathcal{L} = \sup_{s_t(x)}  \inf_{q_t(x)} \; \int dx\; s_1(x) p_1(x) -\int dx\; s_0(x) p_0(x) -  \int \limits_0^1 \int \limits_{\mathcal{X}} dt dx \; q_t(x) \;\bigg[\frac{1}{2} \| \nabla s_t(x) \|^2 + \frac{1}{2}s_t(x)^2 + \deriv{s_t(x)}{t}\bigg].
\end{split}
\end{align}
The first order condition for $q_t$ is
\begin{align}
    \nabla\bigg[\frac{1}{2} \| \nabla s_t(x) \|^2 + \frac{1}{2}s_t(x)^2 + \deriv{s_t(x)}{t}\bigg] = 0.
\end{align}
The first order condition for $s_t$ yields
\begin{align}
    \deriv{q_t(x)}{t} = - \inner{\nabla}{q_t(x)\nabla s_t(x)} + s_t(x)q_t(x), \;\; q_0 = p_0, \;\; q_1 = p_1.
\end{align}
\end{proof}

\subsection{Schrödinger Bridge Problem}\label{app:proofs_sbp}

\begin{proposition*}
This optimization problem
\begin{align}\label{eq:sbp}
    \inf_{q_t,v_t} \int dtdx\; q_t \bigg[\frac{1}{2}\norm{v_t}^2 + \frac{\sigma^4}{8} \norm{\nabla \log q_t}^2\bigg],
    \;\;\text{ s.t. }\;\; \dot{q}_t = -\inner{\nabla}{q_t v_t}, q_0 = p_0, q_1 = p_1\,,
\end{align}
is equivalent to
\begin{align}
\begin{split}
    \mathcal{L} = \sup_{s_t(x)}  \inf_{q_t(x)} \;  \int \limits_0^1 \int \limits_{\mathcal{X}} dt dx \; q_t(x) \;  \bigg[-\frac{1}{2} \| \nabla s_t(x) \|^2 - \frac{\sigma^2}{2} \Delta s_t - \deriv{s_t}{t}\bigg] + \int dx\; s_1(x) p_1(x) -\int dx\; s_0(x) p_0(x)\,.
\end{split}
\end{align}
In the optimum, we have
\begin{align}
    \deriv{q_t(x)}{t} = - \inner{\nabla}{q_t(x)\nabla s_t(x)} + \frac{\sigma^2}{2}\Delta q_t, \;\; q_0 = p_0, \;\; q_1 = p_1, \;\; \text{ and }\;\; \frac{1}{2} \| \nabla s_t(x) \|^2 + \deriv{s_t(x)}{t} + \frac{\sigma^2}{2}\Delta s_t = 0.
\end{align}
\end{proposition*}
\begin{proof}
The Lagrangian of the original optimization problem is
\begin{align}
\begin{split}
    \mathcal{L} = \sup_{s_t(x)}  \inf_{q_t(x)} & \;  \int \limits_0^1 \int \limits_{\mathcal{X}} dt dx \; q_t(x) \;  \bigg[\frac{1}{2} \| v_t(x) \|^2 + \frac{\sigma^4}{8} \norm{\nabla \log q_t}^2\bigg]  + \int \limits_0^1 \int \limits_{\mathcal{X}} dt dx \; \lambda_t(x) \bigg[  \frac{\partial q_t(x) }{\partial t}  + \inner{\nabla}{q_t(x) v_t(x)} \bigg] \\
    & + \int dx\; \lambda_1(x) \bigg( p_1(x) - q_1(x) \bigg) -\int dx\; \lambda_0(x) \bigg( p_0(x) - q_0(x) \bigg).
\end{split}
\end{align}
Optimization w.r.t. $v_t$ yields $v_t = \nabla \lambda_t$, and we rename $\lambda_t$ as $s_t$.
Then in the optimum we have
\begin{align}
    \deriv{q_t(x)}{t} = - \inner{\nabla}{q_t(x)\nabla s_t(x)}, \;\; \text{ and }\;\; \frac{1}{2} \| \nabla s_t(x) \|^2 + \deriv{s_t(x)}{t} = -\frac{\sigma^4}{8}\norm{\nabla \log q_t}^2 - \frac{\sigma^4}{4}\Delta \log q_t.
\end{align}
Note that $s_t = -\frac{\sigma^2}{2} \log q_t$ solves the last equation. 
However, it might not satisfy the boundary conditions.
Let's parameterize then $s_t = \tilde{s}_t -\frac{\sigma^2}{2} \log q_t$.
Then we will end up in the solution
\begin{align}
    \deriv{q_t(x)}{t} = - \inner{\nabla}{q_t(x)\nabla \tilde{s}_t(x)} + \frac{\sigma^2}{2}\Delta q_t, \;\; \text{ and }\;\; \frac{1}{2} \| \nabla \tilde{s}_t(x) \|^2 + \deriv{\tilde{s}_t(x)}{t} + \frac{\sigma^2}{2}\Delta \tilde{s}_t = 0.
\end{align}
We first take some integrals by parts
\begin{align}
\begin{split}
    \mathcal{L} = \sup_{s_t(x)}  \inf_{q_t(x)} & \;  \int \limits_0^1 \int \limits_{\mathcal{X}} dt dx \; q_t(x) \;  \bigg[-\frac{1}{2} \| \nabla s_t(x) \|^2 - \deriv{s_t}{t} + \frac{\sigma^4}{8} \norm{\nabla \log q_t}^2\bigg]  \\
    & + \int dx\; s_1(x) p_1(x) -\int dx\; s_0(x) p_0(x)\,,
\end{split}
\end{align}
and then put $s_t = \tilde{s}_t -\frac{\sigma^2}{2} \log q_t$; whence, we get
\begin{align}
\begin{split}
    \mathcal{L} = \sup_{\tilde{s}_t(x)}  \inf_{q_t(x)} & \;  \int \limits_0^1 \int \limits_{\mathcal{X}} dt dx \; q_t(x) \;  \bigg[-\frac{1}{2} \| \nabla \tilde{s}_t(x) \|^2 + \frac{\sigma^2}{2}\inner{\nabla \tilde{s}_t}{\nabla \log q_t} - \deriv{\tilde{s}_t}{t} + \frac{\sigma^2}{2} \deriv{}{t}\log q_t\bigg]  \\
    & + \int dx\; \tilde{s}_1(x) p_1(x) -\int dx\; \tilde{s}_0(x) p_0(x) - \frac{\sigma^2}{2} \int dx\; p_1(x) \log q_1(x)  + \frac{\sigma^2}{2}\int dx\; p_0(x)\log q_0(x).
\end{split}
\end{align}
Doing integration by parts, we get
\begin{align}
\begin{split}
    \mathcal{L} = \sup_{\tilde{s}_t(x)}  \inf_{q_t(x)} & \;  \int \limits_0^1 \int \limits_{\mathcal{X}} dt dx \; q_t(x) \;  \bigg[-\frac{1}{2} \| \nabla \tilde{s}_t(x) \|^2 - \frac{\sigma^2}{2} \Delta \tilde{s}_t - \deriv{\tilde{s}_t}{t}\bigg]  \\
    & + \int dx\; \tilde{s}_1(x) p_1(x) -\int dx\; \tilde{s}_0(x) p_0(x) - \frac{\sigma^2}{2} \int dx\; p_1(x) \log q_1(x)  + \frac{\sigma^2}{2}\int dx\; p_0(x)\log q_0(x).
\end{split}
\end{align}

This Lagrangian corresponds to the following constrained optimization problem
\begin{align}
\begin{split}
    \inf_{q_t(x), v_t} & \;  \int \limits_0^1 \int \limits_{\mathcal{X}} dt dx \; q_t(x) \frac{1}{2}\norm{v_t}^2 - \frac{\sigma^2}{2} \int dx\; p_1(x) \log q_1(x)  + \frac{\sigma^2}{2}\int dx\; p_0(x)\log q_0(x),\;\; \text{ subj. to}   \\
    & \deriv{q_t(x)}{t} = - \inner{\nabla}{q_t(x)v_t(x)} + \frac{\sigma^2}{2}\Delta q_t,\;\; q_1(x) = p_1(x), \;\;  q_0(x) = p_0(x)\,,
\end{split}
\end{align}
which is equivalent to
\begin{align}
\begin{split}
    \inf_{q_t(x), v_t} & \;  \int \limits_0^1 \int \limits_{\mathcal{X}} dt dx \; q_t(x) \frac{1}{2}\norm{v_t}^2 + \frac{\sigma^2}{2} \KL(p_1(x), q_1(x)) - \frac{\sigma^2}{2} \KL(p_0(x), q_0(x)) ,\;\; \text{ subj. to}   \\
    & \deriv{q_t(x)}{t} = - \inner{\nabla}{q_t(x)v_t(x)} + \frac{\sigma^2}{2}\Delta q_t,\;\; q_1(x) = p_1(x), \;\;  q_0(x) = p_0(x)\,.
\end{split}
\end{align}
Note that the constraints on the end-points marginals zero out the KL-divergences in the objective.
Whence, we have
\begin{align}
\begin{split}
    \inf_{q_t(x), v_t} & \;  \int \limits_0^1 \int \limits_{\mathcal{X}} dt dx \; q_t(x) \frac{1}{2}\norm{v_t}^2,\;\; \text{ subj. to}   \\
    & \deriv{q_t(x)}{t} = - \inner{\nabla}{q_t(x) v_t(x)} + \frac{\sigma^2}{2}\Delta q_t,\;\; q_1(x) = p_1(x), \;\;  q_0(x) = p_0(x)\,,
\end{split}
\end{align}
which dual is
\begin{align}
\begin{split}
    \mathcal{L} = \sup_{s_t(x)}  \inf_{q_t(x)} \;  \int \limits_0^1 \int \limits_{\mathcal{X}} dt dx \; q_t(x) \;  \bigg[-\frac{1}{2} \| \nabla s_t(x) \|^2 - \frac{\sigma^2}{2} \Delta s_t - \deriv{s_t}{t}\bigg] + \int dx\; s_1(x) p_1(x) -\int dx\; s_0(x) p_0(x)\,.
\end{split}
\end{align}
The optimality conditions follow from the differentiation w.r.t. $q_t$ and $s_t$.
\end{proof}
